q-Paths: Generalizing the Geometric Annealing Path using Power Means

Many common machine learning methods involve the geometric annealing path, a sequence of intermediate densities between two distributions of interest constructed using the geometric average. While alternatives such as the moment-averaging path have demonstrated performance gains in some settings, their practical applicability remains limited by exponential family endpoint assumptions and a lack of closed form energy function. In this work, we introduce $q$-paths, a family of paths which is derived from a generalized notion of the mean, includes the geometric and arithmetic mixtures as special cases, and admits a simple closed form involving the deformed logarithm function from nonextensive thermodynamics. Following previous analysis of the geometric path, we interpret our $q$-paths as corresponding to a $q$-exponential family of distributions, and provide a variational representation of intermediate densities as minimizing a mixture of $\alpha$-divergences to the endpoints. We show that small deviations away from the geometric path yield empirical gains for Bayesian inference using Sequential Monte Carlo and generative model evaluation using Annealed Importance Sampling.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> sections/app/breg_table.tex <==
\section{Comparison of Exponential Family and $q$-Exponential Family}\label{app:breg_table}
\begin{table}[h]
\centering
\caption{\label{tab:properties}}
\begin{tabular}{p{2cm} p{6.1cm} p{6.5cm}} % \cmidrule(r){1-1}
  \cmidrule(lr){2-2} \cmidrule(l){3-3} \\[.25ex]
 & Exponential Family ($q=1$) & $q$-Exponential Family \\ \midrule
Definition & $\pi_{\beta}(\z) = \pi_0(\z) \, \exp \{ \beta \cdot \phi(\z) - \psi(\beta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z) \, \exp_q \{ \lambda \cdot \phi(\z) - \psi_q(\lambda) \} $ \\[2ex]
Free Energy & $\psi(\beta)  = \ln Z_{\beta} $ & $\psi_q(\lambda)$ \\[2ex]
Escort Dist. & $\Pi_{\beta, 1} =  \pi_0(\z)^{1-1} \, \pi_{\beta}(\z)^1 =  \pi_{\beta}(\z)  $ & $ \Pi_{\lambda,q} = \dfrac{1}{z_{q}(\lambda)} \pi_0(\z)^{1-q} \, \pi_{\lambda,q}(\z)^q $ \\[2ex]
Dual Params 		& $\dfrac{\partial \psi(\beta)}{\partial \beta^j} = \eta^j =  \mathbb{E}_{\pi_{\beta}}[\phi_j(\z)]$    \, (standard)		& $\dfrac{\partial \psi_q(\lambda)}{\partial \lambda^j} =\eta^j_q =\mathbb{E}_{\Pi_{\lambda,q}}[\phi_j(\z)] $ \, (escort) \\[2ex]
Bregman Div. & $D_{\psi}[\beta^{\prime} : \beta ] = D_{KL}[ \pi_{\beta} || \pi_{\beta^{\prime}} ] $ & $D_{\psi_q}[\lambda^{\prime} : \lambda ] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda,q}}{\pi_0} - \ln_q \dfrac{\pi_{\lambda^{\prime},q}}{\pi_0}] $ \\[2ex]
& $\phantom{D_{\psi}[\beta^{\prime} : \beta ]} = \mathbb{E}_{\pi_{\beta}} [ \ln \pi_{\beta} - \ln \pi_{\beta^{\prime}} ]$ &  \\[2ex]
Conjugate $\psi^{*}$ & $\psi^{*}(\eta) = D_{\psi}[\pi_0 ||  \pi_{\beta_{\eta}}] =D_{KL}[\pi_{\beta_{\eta}}||\pi_0 ] $ & $\psi_q^{*}(\eta) = D_{\psi_q}[\pi_0 ||\pi_{\lambda_{\eta},q}] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda_{\eta},q}}{\pi_0} ] $\\[2ex]
& & $\phantom{\psi_q^{*}(\eta) = } \hfill = \dfrac{1}{1-q}\bigg(\dfrac{1}{z_q(\lambda)} -1 \bigg) $ \\[3.5ex] \\
Neg. Entropy & $\psi^{*}(\eta) = \mathbb{E}_{\pi_{\beta_{\eta}}}[ \log \pi_{\beta_{\eta}} ] $\footnotesize \quad (if $\pi_0 =$uniform)& $\psi_q^{*}(\eta) = \mathbb{E}_{\Pi_{\lambda, q}}[ \ln_q \pi_{\lambda_{\eta},q} ] $  \footnotesize \quad (if $\pi_0 = $uniform) \\[3ex]
\small Dual Definition & $\pi_{\beta}(\z) = \pi_0(\z) \exp \{ \beta \, ( \phi(\z) - \eta ) + \psi^{*}(\eta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z)\exp_q \{ \lambda \, ( \phi(\z) - \eta_q ) + \psi_q(\lambda) \}$ \\
\bottomrule
\end{tabular}
\end{table}


==> sections/app/geo.tex <==
\newcommand{\alphaainv}{{\frac{2}{1-\alpha}}}
\newcommand{\alphaa}{{\frac{1-\alpha}{2}}}
\newcommand{\alphaaneg}{{\frac{1+\alpha}{2}}}
\newcommand{\alphaaneginv}{{\frac{2}{1+\alpha}}}

\section{\citet{zhang2013nonparametric} Geodesics }
This section closely follows \citet{zhang2013nonparametric} Sec. 2.2-2.3.
We will seek to show that our $q$-path
\begin{align}
    \ln_q \big(\tpi_{t, q}(z)\big) = (1-t) \ln_q \big(\tpi_{0}(z)\big) + t \, \ln_q \big(\tpi_{1}(z) \big)
\end{align}
forms a geodesic for the affine connection induced by the $\alpha$-divergence $D_{\alpha}$ over unnormalized measures.


Consider the $\rho, \tau$ embeddings
\begin{align}
    \rho(\tpi(z)) =  \alphaainv \big( \tpi(z)^\alphaa - 1 \big) \qquad \tau(\tpi) = \alphaaneginv  \big( \tpi(z)^\alphaaneg - 1 \big)
\end{align}
which are conjugate with respect to the function
\begin{align}
    f(\rho) = \alphaaneginv \big( 1 + \alphaa \cdot \rho)^\alphaainv
\end{align}
where conjugacy means that $\tau(\tpi(z)) = f^{\prime}\big(\rho(\tpi(z))\big)$.


This induces a family of $\alpha$-divergences $D^{(\alpha)}_{f,\rho}$, where $\alpha$ is intended to reflect \textit{referential duality}.   Our use of $\alpha$ in the $\rho, \tau$ embedding functions, or $q$ in the $\ln_q$ path, rather reflects \textit{representational duality} in terms of the $\alpha$-representation (e.g. \citet{amari2010divergencefunctions}).

% geodesic is wrt second argument
We obtain the flat divergence, which integrates an expression of Bregman form
\begin{align}
    D^{(1)}_{f, \rho}[\tpi_a:\tpi_b] =  \int f\big(\rho(\tpi_a(z)) \big) -  f\big(\rho(\tpi_b(z)) \big) + \big( \rho(\tpi_a(z)) - \rho(\tpi_b(z)) \big) \cdot  \tau(\tpi_b) dz
\end{align}
which can be shown to correspond to Amari's $\alpha$ divergence for the choice of $f, \rho$ above.
\begin{align}
D^{(1)}_{f, \rho}[\tpi_a:\tpi_b] &= D_{\alpha}[\tpi_a(\vz):\tpi_b(\vz) ] \\
&= \frac{4}{(1-\alpha^2)} \bigg( \frac{1-\alpha}{2}  \int \tpi_a(\vz) \,d\vz +  \frac{1+\alpha}{2}  \int \tpi_b(\vz) \,d\vz -\int \tpi_a(\vz)^{\frac{1-\alpha}{2}} \, \tpi_b(\vz)^{\frac{1+\alpha}{2}}  d\vz  \bigg)
\end{align}
As shown in Proposition 2 and Corollary 3 of \citet{zhang2013nonparametric}, we can define an information manifold $(\mathcal{M}_+, g_{ij}^{(D^{(1)}_{f,\rho})}, \nabla^{(1)}, \nabla^{(-1)})$.   See \citet{zhang2013nonparametric} for additional details.   We consider only the affine connection $\nabla^{(1)}$ in what follows, which is a special case of the $\alpha$-connection for the above manifold
\begin{align*}
    \nabla^{(\alpha)}_{\dot{\gamma}} \dot{\gamma} = (d_{\dot{\gamma}} \dot{\gamma})_{\gamma_t} + \frac{d}{d\gamma} \big( \alphaaneg \log \rho^{\prime}(\gamma(t)) + \alphaa \log \tau^{\prime}(\gamma(t)) \big) \label{eq:affine_alpha}
\end{align*}



\subsection{$q$-Path as Geodesic}
Our $q$-path distributions $\tpi_{t, q}$ along a curve parameterized by $t$, are defined using the power mean with function $\rho(u)$, and are thus linear in the $\rho$ representation
\begin{align}
    \rho\big( \gamma(t)\big) = \rho\big(\tpi_{t, q}(z)\big) = (1-t) \rho\big(\tpi_{0}(z)\big) + t \, \rho\big(\tpi_{1}(z) \big)
\end{align}
where $\rho(u) = \ln_q(u)$ for $q = 2\alpha-1$. %(see Eq. \eqref{eq:lnqexpq}).

We seek to show that our $q$-path is a geodesic with respect to the affine connection $\nabla^{(1)}$, or an autoparallel path.  Let $\gamma_t = \gamma(t) = \tpi_{t,q}(z)$ indicate the $q$-path distribution with mixing parameter $t$, with $\dot{\gamma} = d \gamma_t / dt$.

Plugging $\alpha = 1$ into \eqref{eq:affine_alpha} , and with $ (d_{\dot{\gamma}} \dot{\gamma})_{\gamma_t} = \frac{d \dot{\gamma(t)}}{d\gamma_t} \cdot \dot{\gamma}$ , we seek to show that $\nabla_{\dot{\gamma}} \dot{\gamma} = 0$, or
\begin{align*}
    \nabla^{(1)}_{\dot{\gamma}} \dot{\gamma} = \frac{d \dot{\gamma}}{d\gamma} \cdot \dot{\gamma} + \big(\dot{\gamma}\big)^{2} \cdot \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big)
\end{align}


We will first derive several useful quantities.  Since it is easier to differentiate $\rho(\gamma(t)) = (1-t) \rho(\pi_0) + t \, \rho(\tpi_1)$ with respect to $\gamma$, we note that $\frac{d}{dt} \rho\big( \gamma(t) \big) = \frac{d \rho(\gamma) }{d\gamma(t)} \frac{d\gamma(t)}{dt}$.  We can then rewrite the desired $\frac{d\gamma(t)}{dt}$ as
\begin{align}
    \dot{\gamma} = \frac{d\gamma(t)}{dt} &= \bigg( \frac{d \rho(\gamma_t) }{d\gamma(t)} \bigg)^{-1} \, \frac{d \rho(\gamma_t) }{dt} = \gamma^{\alphaaneg} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \\[1.4ex]
    \implies  \dot{\gamma} &=\gamma_t \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \quad (\text{for $\alpha = 1$}) \label{eq:dgamma_dt}
\end{align}
since
\begin{align}
    \frac{d \rho(\gamma_t) }{d\gamma_t}  &= \frac{d}{d \gamma_t} \alphaainv \big( \gamma^\alphaa - 1 \big) = \gamma_t^{\alphaa - \frac{2}{2}} =  \gamma_t^{\frac{-(1+\alpha)}{2}} \\
    \text{and } \quad \frac{d \rho(\gamma_t) }{dt}  &= \frac{d}{dt} \big( (1-t) \rho(\pi_0) + t \, \rho(\tpi_1) \big) = \rho(\tpi_1) - \rho(\pi_0)
\end{align}

We can now differentiate the $\frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) $ term in the affine connection.   From above, $d \rho(\gamma_t) / d\gamma(t) = \gamma_t^{\frac{-(1+\alpha)}{2}}$, so that
\begin{align}
    \frac{d}{d\gamma} \big(  \log \frac{d}{d\gamma} \rho(\gamma(t)) \big) &=   \frac{d}{d\gamma}   \log \big( \gamma_t^{\frac{-(1+\alpha)}{2}} \big) = -\frac{(1+\alpha)}{2} \cdot \frac{d}{d\gamma}   \log \gamma_t \\
    &\phantom{\frac{d}{d\gamma}   \log \big( \gamma_t^{\frac{-(1+\alpha)}{2}} \big)} = -\frac{(1+\alpha)}{2} \gamma_t^{-1} \\
    % &= \gamma_t^{\frac{(1+\alpha)}{2}} \cdot \frac{d}{d\gamma} \gamma_t^{\frac{(1+\alpha)}{2}} \\
    % % &=
    % % \bigg( \frac{d}{d\gamma} \rho(\gamma_t) \bigg)^{-1} \cdot \frac{d}{d\gamma}  \rho(\gamma_t) \\
    % &= \gamma^{\frac{(1+\alpha)}{2}} \cdot  - \frac{(1+\alpha)}{2} \gamma^{-\frac{(1+\alpha)}{2}-1} \\
    % &= -\gamma_t \cdot \gamma_t^{-2} \\
    \implies \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) &=  -\gamma_t^{-1} \quad (\text{for $\alpha=1$}) \label{eq:db_dgamma}
\end{align}


Putting it all together, and with dot products turning into scalar products for our one-dimensional curve $t$, we have
\begin{align}
    \nabla^{(1)}_{\dot{\gamma}} \dot{\gamma} &=  \frac{d \dot{\gamma}}{d\gamma_t} \cdot \dot{\gamma}  + \big(\dot{\gamma}\big)^{2} \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) \\
    &=  \frac{d }{d\gamma_t} \bigg( \gamma_t \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \bigg) \cdot \dot{\gamma}  -  (\dot{\gamma})^{2} \gamma_t^{-1}
    \qquad \quad \text{(using \eqref{eq:dgamma_dt} and \eqref{eq:db_dgamma})} \\
    &= \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) - (\dot{\gamma})^{2} \cdot {\dot{\gamma}}^{-1} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \qquad \text{(rearranging \eqref{eq:dgamma_dt})} \\
    &= \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) - \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \\
    &=0
\end{align}

\clearpage
\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_09.pdf}}
    \subfigure[$q=0.9$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_18.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_20.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_12_redo.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_2_redo.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_3_redo.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_4_redo.pdf}}
    \caption{Intermediate densities between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$ for various $q$-paths and 10 equally spaced $\beta$. The path approaches a mixture of Gaussians with  weight $\beta$ at $q=0$.  For the geometric mixture ($q=1$), intermediate $\pi_{\beta}$ stay within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:alpha_path}
    \vspace*{-.15cm}
\end{figure}


\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha-1_student_df2_2.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha05_student_df2_2.pdf}}
    \subfigure[$q=0.95$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha95_student_df2_2.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha1_student_df2_2.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha11_student_df2_2.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha15_student_df2_2.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha2_student_df2_2.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha3_student_df2_2.pdf}}
    \caption{Intermediate densities between $\text{Student}(\text{df}=2, -4, 3)$ and $\text{Student}(\text{df}=2, 4, 1)$ for various $q$-paths and 10 equally spaced $\beta$.}
    \label{fig:q_path}
    \vspace*{-.15cm}
\end{figure}



\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha-1_student_df2_2.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha05_student_df2_2.pdf}}
    \subfigure[$q=0.95$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha95_student_df2_2.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha1_student_df2_2.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha11_student_df2_2.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha15_student_df2_2.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha2_student_df2_2.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha3_student_df2_2.pdf}}
    \caption{Tail behavior for densities between $\text{Student}(\text{df}=2, -4, 3)$ and $\text{Student}(\text{df}=2, 4, 1)$ for various $q$-paths and 10 equally spaced $\beta$.}
    \label{fig:q_path}
    \vspace*{-.15cm}
\end{figure}


==> sections/app/old/app.tex <==
\section{Abstract Mean is Invariant to Affine Transformations} \label{app:any_h}
In this section, we show that $h_{q}(u)$ is invariant to affine transformations. That is, for any choice of $a$ and $b$,
\begin{align}
    h_{q}(u) =
\begin{cases}
    a \cdot u^{1-q} + b \hfill & q \neq 1 \\
    \log u \hfill 	&  q = 1
\end{cases} \label{eq:alpha_abstract2}
\end{align}
yields the same expression for the abstract mean $\mu_{h_{\alpha}}$. First, we note the expression for the inverse $h^{-1}_{q}(u)$ at $q \neq 1$
\begin{align}
    h^{-1}_{q}(u) = \left(\frac{u - b}{a}\right)^{\frac{1}{1-q}}.
\end{align}
Recalling that $\sum_i w_i = 1$, the abstract mean then becomes
\begin{align}
    \mu_{h_{q}}(\{w_i\}, \{u_i\}) &= h_{q}^{-1}\left(\sum_i w_i h_{q}(u_i) \right) \\
    &= h_{q}^{-1}\left(a \left(\sum_i w_iu_i^{1-q}\right) + b \right) \\
    &=\bigg(\sum_i w_i u_i^{1-q} \bigg)^{\frac{1}{1-q}}
\end{align}
which is independent of both $a$ and $b$.
%The $\alpha$-representation \cite{amari2007integration,amari2016information} appears as a special case with $a=1$ and $b=0$, while the deformed logarithm $\ln_q$ corresponds to $a=-b = \frac{1}{1-q}$ for $q=\frac{1+\alpha}{2}$.

\section{Derivations of the $q$-Path}\label{app:q_path}
\subsection{Deformed Log Mixture}\label{app:ln_qmix}
In this section, we show that the unnormalized $\ln_q$ mixture
\begin{align}
\ln_q \tpi^{(q)}_{\beta}(\z) &=  (1-\beta) \ln_q \pi_0(\z) + \beta \ln_q \tpi_1(\z)
\end{align}
reduces to the form of the $q$-path intermediate distribution in \eqref{qpath_mix_form} and \eqref{eq:alpha_mix}.  Taking $\exp_q$ of both sides,
\begin{align*}
    \tpi^{(q)}_{\beta}(\z) &=  \exp_q \left\{ (1-\beta) \ln_q \pi_0(\z) + \beta \ln_q \tpi_1(\z)  \right\} \\
    &= \left[ 1 + (1-q) \left( \ln_q \pi_0(\z) + \beta \left( \ln_q \tpi_1(\z) - \ln_q \pi_0(\z) \right)\right) \right]_{+}^{\frac{1}{1-q}} \\
    &= \left[ 1 + (1-q) \frac{1}{1-q} \left( \pi_0(\z)^{1-q} - 1  + \beta \big( \tpi_1(\z)^{1-q} - 1 - \pi_0(\z)^{1-q} + 1 \big)\right)   \right]_{+}^{\frac{1}{1-q}} \\
  &= \left[ 1 +  \pi_0(\z)^{1-q} - 1  + \beta \bigg( \tpi_1(\z)^{1-q}  - \pi_0(\z)^{1-q} \bigg) \right]_{+}^{\frac{1}{1-q}} \\
  &= \left[  \pi_0(\z)^{1-q}  + \beta \, \tpi_1(\z)^{1-q} - \beta \, \pi_0(\z)^{1-q}    \right]_{+}^{\frac{1}{1-q}} \\
  &= \left[  (1-\beta ) \, \pi_0(\z)^{1-q}  + \beta \, \tpi_1(\z)^{1-q}  \, \right]_{+}^{\frac{1}{1-q}}
\end{align*}

\subsection{$q$-Exponential Family}\label{app:qexp_derivation}
Here, we show that the unnormalized $q$-path reduces to a form of the $q$-exponential family
%\begin{proof}
\begin{align}
    \tilde{\pi}_{\beta, q} &= \bigg[(1 - \beta) \pi_0(\vz)^{1 - q} + \beta \tpi_1(\vz)^{1 - q}\bigg]^\frac{1}{1 - q}\\
    &= \bigg[\pi_0(\vz)^{1 - q} + \beta\big(\tpi_1(\vz)^{1 - q} - \pi_0(\vz)^{1 - q}\big)\bigg]^\frac{1}{1 - q}\\
    &= \pi_0(\vz) \left[1 + \beta\left(\left(\frac{\tpi_1(\vz)}{\pi_0(\vz)}\right)^{1 - q} - 1\right)\right]^\frac{1}{1 - q}\\
    &= \pi_0(\vz) \left[1 + (1-q) \, \beta \, \ln_q\left( \frac{\tpi_1(\vz)}{\pi_0(\vz)}\right)\right]^\frac{1}{1 - q}\\
    &= \pi_0(\vz) \exp_q \left\{ \beta \cdot \ln_q\left(\frac{\tpi_1(\vz)}{\pi_0(\vz)}\right)\right\}.
\end{align}
Defining $\phi(\vz) = \ln_{q} \frac{\tpi_1(\vz)}{\pi_0(\z)}$ and introducing a multiplicative normalization factor $Z_q(\beta)$, we arrive at
\begin{align}
    \pi^{(q)}_{\beta}(z) = \frac{1}{Z_q(\beta)} \, \pi_0(\vz)\exp_q \left\{\beta \cdot  \phi(\vz) \right\} \qquad
    Z_q(\beta) &:= \int  \pi_0(\vz) \exp_q \left\{ \beta \cdot \phi(\vz)\right\} \, d\vz .\label{eq:lnq_fam_form2}
\end{align}

\subsection{Normalization in q-Exponential Families}\label{app:normalization}
%\section{Alternative Derivation}
The $q$-exponential family can also be written using the $q$-free energy $\psi_q(\theta)$ for normalization \cite{amari2011q, naudts2011generalised},
\begin{align}
    \pi_{\theta}^{(q)}(\z)  &= \pi_0(z) \, \exp_q \big\{ \theta \cdot \phi(\vz) - \psi_q(\theta ) \big\} \, . \label{eq:qexp_fam_qf} %\propto \pi_0(z) \, \exp_q \big\{ \lambda \cdot \phi(\vz)  \big\}  % \frac{1}{Z^{(q)}(\lambda)}
\end{align}
However, since $\exp_q \{ x + y \} = \exp_q \{ y \} \cdot \exp_q \{ \frac{x}{1 + (1-q) y}  \}$ (see \cite{suyari2020advantages} or App. \ref{app:q_sum_product} below) instead of $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $ for the standard exponential, we can not easily move between these ways of writing the $q$-family \cite{matsuzoe2019normalization}.

Mirroring the derivations of \citet{naudts2011generalised} pg. 108, we can rewrite \eqref{eq:qexp_fam_qf} using the above identity for $\exp_q \{ x+y\}$, as
\begin{align}
\pi^{(q)}_{\theta}(\vz) &= \pi_0(\vz) \, \exp_q \{ \theta \cdot \phi(\vz) - \psi_q(\theta) \} \label{eq:normalization1} \\
&= \pi_0(\vz) \, \exp_q \{ - \psi_q(\theta) \} \exp_q \big\{ \frac{\theta \cdot \phi(\vz)}{1+(1-q)(-\psi_q(\theta))} \big \} \label{eq:normalization2}
\end{align}
Our goal is to express $\pi^{(q)}_{\theta}(\vz)$ using a normalization constant $Z^{(q)}_\beta$ instead of the $q$-free energy $\psi_q(\theta)$.  While the exponential family allows us to freely move between $\psi(\theta)$ and $\log Z_{\theta}$, we must adjust the natural parameters (from $\theta$ to $\beta$) in the $q$-exponential case.   Defining
%To (w/ $\eta, \beta$ switched) match Naudts, let : }
\begin{align}
 \beta &= \frac{\theta}{1+(1-q)(-\psi_q(\theta))} \\
Z^{(q)}_\beta &= \frac{1}{\exp_q \{-\psi_q(\theta) \}} %:= \exp_{q}^{*}\{ \psi_q(\theta)\} \, ,
\end{align}
we can obtain a new parameterization of the $q$-exponential family, using parameters $\beta$ and multiplicative normalization constant $Z^{(q)}_\beta$,
\begin{align}
 \pi^{(q)}_{\beta}(\vz) &=  \frac{1}{Z^{(q)}_\beta} \pi_0(z) \, \exp_{q} \{ \beta \cdot \phi(\vz) \} \\
 &= \pi_0(z) \, \exp_q \big\{ \theta \cdot \phi(\vz) - \psi_q(\theta ) \big\} = \pi^{(q)}_{\theta}(\vz)  \, .
\end{align}
See \citet{matsuzoe2019normalization}, \citet{suyari2020advantages}, and \citet{naudts2011generalised} for more detailed discussion of normalization in deformed exponential families.


\section{Minimizing $\alpha$-divergences}\label{app:alpha_integration}
\citet{amari2007integration} shows that the $\alpha$ power mean $\pi^{(\alpha)}_{\beta}$ minimizes the expected divergence to a single distribution, for \textit{normalized} measures and $\alpha = 2q-1$.   We repeat similar derivations but for the case of unnormalized endpoints $\{\tpi_i\}$ and $\tilde{r}(\vz)$
\begin{align}
\tpi_{\alpha}(\vz) &= \argmin \limits_{\tilde{r}(\vz)} \sum \limits_{i=1}^{N} w_i \, D_{\alpha}[\tpi_i (\vz) : \tilde{r}(\vz) ] \label{eq:amari_vrep} \\
\text{where} \quad \tpi_{\alpha}(\vz) &= \big( \sum \limits_{i=1}^{N} w_i \, \tpi_i (\vz)^{\frac{1-\alpha}{2}}     \big)^{\frac{2}{1-\alpha}} \label{eq:alpha_mix_app}
\end{align}
\begin{proof}
\begin{align}
\frac{d}{d\tilde{r}} \sum \limits_{i=1}^{N} w_i \, D_{\alpha}[\tpi_i (\vz) : \tilde{r}(\vz) ] &= \frac{d}{d\tilde{r}} \frac{4}{1-\alpha^2} \sum \limits_{i=1}^{N} w_i \big( -\int \tpi_i(\vz)^{\frac{1-\alpha}{2}}\, \tilde{r}(\vz)^{\frac{1+\alpha}{2}} d\vz  +  \frac{1+\alpha}{2} \int \tilde{r}(\vz) d\vz \big) \\
0 &=\frac{4}{1-\alpha^2} \big( -{\frac{1+\alpha}{2}} \sum \limits_{i=1}^{N} w_i  \, \tpi_i(\vz)^{\frac{1-\alpha}{2}}\, \tilde{r}(\vz)^{\frac{1+\alpha}{2}-1} + \frac{1+\alpha}{2} \big) \\
- \frac{2}{1-\alpha} &= -\frac{2}{1-\alpha} \sum \limits_{i=1}^{N} w_i  \, \tpi_i(\vz)^{\frac{1-\alpha}{2}}  \tilde{r}(\vz)^{-\frac{1-\alpha}{2}} \\
 \tilde{r}(\vz)^{\frac{1-\alpha}{2}} &= \sum \limits_{i=1}^{N} w_i  \, \tpi_i(\vz)^{\frac{1-\alpha}{2}} \\
  \tilde{r}(\vz) &= \bigg(\sum \limits_{i=1}^{N} w_i  \, \tpi_i(\vz)^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
\end{align}
\end{proof}
%The function $f_{\alpha}(p) = \frac{2}{1-\alpha} \, p^{\frac{1-\alpha}{2}}$ is known as the $\alpha$-representation of a distribution $p$ \cite{amari2016information}.
This result is similar to a general result about Bregman divergences in \citet{Banerjee2005} Prop. 1. although $D_{\alpha}$ is not a Bregman divergence over normalized distributions.


% While the $\alpha$-integration of \citet{amari2007integration} corresponds to our $q$-paths, except for the case of normalized distributi
\subsection{Arithmetic Mean ($q=0$)}\label{app:mixture_path}
\newcommand{\pa}{\pi_0}%{p_a}
\newcommand{\pb}{\pi_1}%{p_b}
\newcommand{\opt}{r}%{q}
%\section{Relationship between \texorpdfstring{$\alpha$}{}-mean path and Grosse's moment averaging path}\label{app:grosse_alpha
For normalized distributions, we note that the moment-averaging path from \citet{grosse2013annealing} is \textit{not} a special case of the $\alpha$-integration \cite{amari2007integration}.   While both minimize a convex combination of reverse \textsc{kl} divergences, \citet{grosse2013annealing} minimize within the constrained space of exponential families, %\textit{minimal exponential families}
 while \citet{amari2007integration} optimizes over \textit{all} normalized distributions.

More formally, consider minimizing the functional
\begin{align}
    J[\opt] &= (1 - \beta)\int \pa(z) \log \frac{\pa(z)}{\opt(z)} dz + \beta \int \pb(z) \log \frac{\pb(z)}{\opt(z)} dz \\
         &= \text{const} - \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \log \opt(z) dz \label{eq:functional}
\end{align}
We will show how \citet{grosse2013annealing} and \citet{amari2007integration} minimize \eqref{eq:functional}.



%\paragraph{Grosse's solution}
\paragraph{Solution within Exponential Family}
\citet{grosse2013annealing} constrains $\opt(z) = \frac{1}{Z(\theta)} h(z) \exp (\theta^T g(z))$ to be a (minimal) exponential family model and minimizes \eqref{eq:functional} w.r.t $\opt$'s  natural parameters $\theta$ (cf. \cite{grosse2013annealing} Appendix 2.2):
\begin{align}
    \theta^*_i &= \argmin_\theta J(\theta) \\
    &= \argmin_\theta \left(- \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \left[ \log h(z) + \theta^T g(z) - \log Z(\theta) \right] dz \right)\\
    &= \argmin_\theta \left(\log Z(\theta) - \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \theta^T g(z) dz  + \text{const}\right)
\end{align}
where the last line follows because $\pa(z)$ and $\pb(z)$ are assumed to be correctly normalized. Then to arrive at the moment averaging path, we compute the partials $\frac{\partial J(\theta)}{\partial \theta_i}$ and set to zero:
\begin{align}
    \frac{\partial J(\theta)}{\partial \theta_i} &= \E_{\opt}[g_i(z)] - (1 - \beta)\E_{\pa}[g_i(z)] - \beta \E_{\pb}[g_i(z)] = 0 \\
    \E_{\opt}[g_i(z)] &= (1 - \beta)\E_{\pa}[g_i(z)] - \beta \E_{\pb}[g_i(z)]
\end{align}
where we have used the exponential family identity $\frac{\partial \log Z(\theta)}{\partial \theta_i} = \E_{\opt_{\theta}}[g_i(z)]$ in the first line.



\paragraph{General Solution}
%\paragraph{Amari's solution}
Instead of optimizing in the space of minimal exponential families, \citet{amari2007integration} instead adds a Lagrange multiplier to \eqref{eq:functional} and optimizes $\opt$ directly (cf. \cite{amari2007integration} eq. 5.1 - 5.12)
\begin{align}
    {\opt}^* &= \argmin_{\opt} J'[\opt] \\
    &= \argmin_{\opt} J[\opt] + \lambda \left(1 - \int \opt(z) dz\right) \label{eq:lagrange}
\end{align}
\cref{eq:lagrange} can be minimized using the Euler-Lagrange equations or using the identity
\begin{align}
    \frac{\delta f(x)}{\delta f(x')} = \delta(x - x')\label{eq:delta_eq}
\end{align}
from \cite{meng2004introduction}. We compute the functional derivative of $J'[\opt]$ using \eqref{eq:delta_eq} and solve for $r$:
\begin{align}
    \frac{\delta J'[\opt]}{\delta \opt(z)}=&- \int \big[(1 - \beta) \pa(z') + \beta \pb(z') \big] \frac{1}{\opt(z')} \frac{\delta \opt(z')}{\delta \opt(z)} dz' - \lambda \int \frac{\delta \opt(z')}{\delta \opt(z)} dz' \\
    =&- \int \big[(1 - \beta) \pa(z') + \beta \pb(z') \big] \frac{1}{\opt(z')} \delta(z - z') dz' - \lambda \int \delta(z - z') dz' \\
    =&- \big[(1 - \beta)\pa(z) + \beta \pb(z)\big] \frac{1}{\opt(z)} - \lambda = 0
\end{align}
Therefore
\begin{align}
    \opt(z) \propto \big[(1 - \beta)\pa(z) + \beta \pb(z)\big],
\end{align}
which corresponds to our $q$-path at $q=0$, or $\alpha = -1$ in \citet{amari2007integration}.  Thus, while both \citet{amari2007integration} and \citet{grosse2013annealing} start with the same objective, they arrive at different optimum because they optimize over different spaces.

\section{Sum and Product Identities for $q$-Exponentials}\label{app:q_sum_product}
In this section, we prove two lemmas which are useful for manipulation expressions involving $q$-exponentials, for example in moving between \cref{eq:normalization1} and \cref{eq:normalization2} in either direction.
\begin{lemma}
    Sum identity
    \begin{align}
        \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
    \end{align}
    \label{lemma:q_exp_sum}
\end{lemma}
\begin{lemma}
    Product identity
    \begin{align}
        \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
    \end{align}
    \label{lemma:q_exp_prod}
\end{lemma}

\subsection{Proof of \cref{lemma:q_exp_sum}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
    \begin{align}
        \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \left[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \right]_{+}^{1/(1-q)} \\
                                                &= \left[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \right]_{+}^{1/(1-q)} \\
                                                &= \left[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \right]_{+}^{1/(1-q)} \\
                                                &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
                                                &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
    \end{align}
\end{proof}
\subsection{Proof of \cref{lemma:q_exp_prod}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + = (1 - q)x_i\right)$. Then,
    %and $(1-q) = (1 - q)$. Then
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
    &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \hspace*{-.5cm} \text{(reindex $n \to n - 1)$} \nonumber \\
    &=\exp_q(x_{0})\exp_q(y_N) & \hspace*{-.5cm} \text{(inductive hypothesis)} \nonumber \\
    &= \bigg[\left(1 + (1-q) \cdot x_{0}\right)\left(1 + (1-q) \cdot y_N\right) \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \cdot x_{0} + \big(1 + (1-q) \cdot x_{0} \big)(1-q) \cdot y_N \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \bigg(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\bigg) \bigg]_{+}^{1/(1-q)}\\
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\right)
\end{align}
Next we use the definition of $y_N$ and rearrange
\begin{align}
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)\left(x_1 + x_2(1 + (1-q) \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + (1-q) \cdot x_i)\right)\right) \nonumber\\
    &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q) x_i\right)\right).
\end{align}
Then reindexing $n \to n + 1$ establishes
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q)x_i\right)\right).
\end{align}
\end{proof}

% % % % \section{Bregman Information (Jensen Gaps \citet{Banerjee2005}}\label{app:breg_info}

% % % \section{The Abstract Mean is Invariant to Affine Transformations in $h_{\alpha}(u)$ } \label{app:any_h}
% % % In this section, we show that any choice of $a$ and $b$ for $h_{\alpha}(u)$ \eqref{eq:alpha_abstract} yields the same expression for the abstract mean $\mu_{h_{\alpha}}$. First, we note the expression for the inverse $h^{-1}_{\alpha}(y)$ at $\alpha \neq 1$
% % % \begin{align}
% % %     h^{-1}_{\alpha}(u) = \left(\frac{u - b}{a}\right)^{\frac{2}{1-\alpha}}.
% % % \end{align}
% % % Recalling that $\sum_i w_i = 1$, the abstract mean then becomes
% % % \begin{align}
% % %     \mu_{h_{\alpha}}(\{w_i\}, \{u_i\}) &= h_{\alpha}^{-1}\left(\sum_i w_i h_{\alpha}(u_i) \right) \\
% % %     &= h_{\alpha}^{-1}\left(a \left(\sum_i w_iu_i^{\frac{1-\alpha}{2}}\right) + b \right) \\
% % %     &=\bigg(\sum_i w_i u_i^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
% % % \end{align}
% % % which is independent of both $a$ and $b$.
% % % The $\alpha$-representation \cite{amari2007integration,amari2016information} appears as a special case with $a=1$ and $b=0$, while the deformed logarithm $\ln_q$ corresponds to $a=-b = \frac{1}{1-q}$. For the abstract mean of two unnormalized densities $\{ f_0, f_T \}$ with weights $\{ 1-t, t \}$, we obtain the $\alpha$-mean in \eqref{qpath_mix_form}.

% % % % prev
% % % % \begin{align}
% % % %     y = h_{\alpha}(u) &= a \cdot u^{\frac{1-\alpha}{2}} + b \\
% % % %     \frac{y - b}{a} &= u^{\frac{1-\alpha}{2}} \\
% % % % \end{align}




% % % \prev
% % \section{Derivations of the $q$-Path}\label{app:q_path}
% % \subsection{Deformed Log Mixture}\label{app:ln_qmix}
% % In this section, we show that the unnormalized $\ln_q$ mixture
% % \begin{align}
% % \ln_q \tpi^{(q)}_{\beta}(\z) &=  (1-\beta) \ln_q \pi_0(\z) + \beta \ln_q \pi_1(\z)
% % \end{align}
% % reduces to the form of the $q$-path intermediate distribution in \eqref{qpath_mix_form} and \eqref{eq:alpha_mix}.  Taking $\exp_q$ of both sides,
% % \begin{align*}
% %     \tpi^{(q)}_{\beta}(\z) &=  \exp_q \left\{ (1-\beta) \ln_q \pi_0(\z) + \beta \ln_q \pi_1(\z)  \right\} \\
% %     &= \left[ 1 + (1-q) \left( \ln_q \pi_0(\z) + \beta \left( \ln_q \pi_1(\z) - \ln_q \pi_0(\z) \right)\right) \right]_{+}^{\frac{1}{1-q}} \\
% %     &= \left[ 1 + (1-q) \frac{1}{1-q} \left( \pi_0(\z)^{1-q} - 1  + \beta \big( \pi_1(\z)^{1-q} - 1 - \pi_0(\z)^{1-q} + 1 \big)\right)   \right]_{+}^{\frac{1}{1-q}} \\
% %   &= \left[ 1 +  \pi_0(\z)^{1-q} - 1  + \beta \bigg( \pi_1(\z)^{1-q}  - \pi_0(\z)^{1-q} \bigg) \right]_{+}^{\frac{1}{1-q}} \\
% %   &= \left[  \pi_0(\z)^{1-q}  + \beta \, \pi_1(\z)^{1-q} - \beta \, \pi_0(\z)^{1-q}    \right]_{+}^{\frac{1}{1-q}} \\
% %   &= \left[  (1-\beta ) \, \pi_0(\z)^{1-q}  + \beta \, \pi_1(\z)^{1-q}  \, \right]_{+}^{\frac{1}{1-q}}
% %     % &= \left[  \pi_0(\z)^{1-q} \left(1 +  t \, \bigg(\frac{\pi_1(\z)}{\pi_0(\z)}\bigg)^{1-q} - t  \right)    \right]_{+}^{\frac{1}{1-q}} \\
% %     % &= \pi_0(\z) \left[ 1 +  (1-q)  \cdot \left( t \cdot \ln_q \frac{\pi_1(\z)}{\pi_0(\z)}  \right) \right]_{+}^{\frac{1}{1-q}} \\
% %     % &= \pi_0(z) \, \exp_q \big\{ \beta_ t \cdot \ln_q \frac{\pi_1(\z)}{\pi_0(\z)}  \big\}
% % \end{align*}
% % % While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \}  $, this is not true for $\exp_{\alpha}\{ x + y \}$.  The $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
% % % \begin{align}
% % %     \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ t \cdot \phi(\vz) - \psi_q  \big\} \label{eq:lnq_fam}
% % % \end{align}
% % % where $\psi_q$ enforces the normalization.  As \citet{amari2011q} show that $\psi_q(t)$ is convex in the parameter $t$, we can write \eqref{eq:lnq_fam} in a form suggestive of the conjugate function $\psi_q^{*}$,
% % % \begin{align}
% % %     \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  t \cdot \phi(\vz) - \psi_q(t) \, .
% % % \end{align}
% % % We now derive the $q$-exponential family from the $\ln_q$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.
% % \subsection{$q$-Exponential Family}\label{app:qexp_derivation}
% % Here, we show that the unnormalized $q$-path reduces to a form of the $q$-exponential family
% % %\begin{proof}
% % \begin{align}
% %     \tilde{\pi}_{\beta, q} &= \bigg[(1 - \beta) \pi_0(\vz)^{1 - q} + \beta \pi_1(\vz)^{1 - q}\bigg]^\frac{1}{1 - q}\\
% %     &= \bigg[\pi_0(\vz)^{1 - q} + \beta\big(\pi_1(\vz)^{1 - q} - \pi_0(\vz)^{1 - q}\big)\bigg]^\frac{1}{1 - q}\\
% %     &= \pi_0(\vz) \left[1 + \beta\left(\left(\frac{\pi_1(\vz)}{\pi_0(\vz)}\right)^{1 - q} - 1\right)\right]^\frac{1}{1 - q}\\
% %     &= \pi_0(\vz) \left[1 + (1-q) \, \beta \, \ln_q\left( \frac{\pi_1(\vz)}{\pi_0(\vz)}\right)\right]^\frac{1}{1 - q}\\
% %     &= \pi_0(\vz) \exp_q \left\{ \beta \cdot \ln_q\left(\frac{\pi_1(\vz)}{\pi_0(\vz)}\right)\right\}.
% % \end{align}
% % Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\vz)}{\pi_0(\z)}$ and introducing a multiplicative normalization factor $Z_q(\beta)$, we arrive at
% % \begin{align}
% %     \pi^{(q)}_{\beta}(z) = \frac{1}{Z_q(\beta)} \, \pi_0(\vz)\exp_q \left\{\beta \cdot  \phi(\vz) \right\} \qquad
% %     Z_q(\beta) &:= \int  \pi_0(\vz) \exp_q \left\{ \beta \cdot \phi(\vz)\right\} \, d\vz .\label{eq:lnq_fam_form2}
% % \end{align}

% % \subsection{Normalization in $q$-Exponential Families}\label{app:normalization}
% % %\section{Alternative Derivation}
% % The $q$-exponential family can also be written using the $q$-free energy $\psi_q(\theta)$ for normalization \cite{amari2011q, naudts2011generalised},
% % \begin{align}
% %     \pi_{\theta}^{(q)}(\z)  &= \pi_0(z) \, \exp_q \big\{ \theta \cdot \phi(\vz) - \psi_q(\theta ) \big\} \, . \label{eq:qexp_fam_qf} %\propto \pi_0(z) \, \exp_q \big\{ \lambda \cdot \phi(\vz)  \big\}  % \frac{1}{Z^{(q)}(\lambda)}
% % \end{align}
% % However, since $\exp_q \{ x + y \} = \exp_q \{ y \} \cdot \exp_q \{ \frac{x}{1 + (1-q) y}  \}$ (see \cite{suyari2020advantages} or App. \ref{app:q_sum_product} below) instead of $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $ for the standard exponential, we can not easily move between these ways of writing the $q$-family \cite{matsuzoe2019normalization}.

% % Mirroring the derivations of \citet{naudts2011generalised} pg. 108, we can rewrite \eqref{eq:qexp_fam_qf} using the above identity for $\exp_q \{ x+y\}$, as
% % \begin{align}
% % \pi^{(q)}_{\theta}(\vz) &= \pi_0(\vz) \, \exp_q \{ \theta \cdot \phi(\vz) - \psi_q(\theta) \} \\
% % &= \pi_0(\vz) \, \exp_q \{ - \psi_q(\theta) \} \exp_q \big\{ \frac{\theta \cdot \phi(\vz)}{1+(1-q)(-\psi_q(\theta))} \big \}
% % \end{align}
% % Our goal is to express $\pi^{(q)}_{\theta}(\vz)$ using a normalization constant $Z^{(q)}_\beta$ instead of the $q$-free energy $\psi_q(\theta)$.  While the exponential family allows us to freely move between $\psi(\theta)$ and $\log Z_{\theta}$, we must adjust the natural parameters (from $\theta$ to $\beta$) in the $q$-exponential case.   Defining
% % %To (w/ $\eta, \beta$ switched) match Naudts, let : }
% % \begin{align}
% %  \beta &= \frac{\theta}{1+(1-q)(-\psi_q(\theta))} \\
% % Z^{(q)}_\beta &= \frac{1}{\exp_q \{-\psi_q(\theta) \}} := \exp_{q}^{*}\{ -\psi_q(\theta)\} \, ,
% % \end{align}
% % we can obtain a new parameterization of the $q$-exponential family, using parameters $\beta$ and multiplicative normalization constant $Z^{(q)}_\beta$,
% % \begin{align}
% %  \pi^{(q)}_{\beta}(\vz) &=  \frac{1}{Z^{(q)}_\beta} \pi_0(z) \, \exp_{q} \{ \beta \cdot \phi(\vz) \} \\
% %  &= \pi_0(z) \, \exp_q \big\{ \theta \cdot \phi(\vz) - \psi_q(\theta ) \big\} = \pi^{(q)}_{\theta}(\vz)  \, .
% % \end{align}
% % See \citet{matsuzoe2019normalization}, \citet{suyari2020advantages}, and \citet{naudts2011generalised} for more detailed discussion of normalization in deformed exponential families.

% % \subsection{Sum Identity for $q$-Exponential}\label{app:q_sum_product}
% % \begin{lemma}
% %     Sum identity
% %     \begin{align}
% %         \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
% %     \end{align}
% %     \begin{proof}
% %         The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
% %         \begin{align}
% %             \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \bigg]^{1/(1-q)} \\
% %                                                     &= \bigg[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \bigg]^{1/(1-q)} \\
% %                                                     &= \bigg[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \bigg]^{1/(1-q)} \\
% %                                                     &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
% %                                                     &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
% %         \end{align}
% %     \end{proof}
% % \end{lemma}

% % %\clearpage
% % % \subsection{Normalization from $\ln_q$ Mixture}\label{app:lnq_norm}
% % % In the case of the standard exponential, the $\log$ mixture can be normalized by subtracting a constant $c = \log Z_{\beta}$.  In general, we might like to write
% % % \begin{align}
% % %     \ln_q \pi^{(q)}_t(\vz) = (1-\beta_t) \, \ln_q \pi_0(\vz) + \beta_t \ln_q \tpi_1(\vz)  - c \, ,  \label{eq:ln_q_mix22}
% % % \end{align}
% % % To normalize by subtracting the $q$-free energy $\psi_q$, we must also multiply by a factor of $\pi_0(\vz)^{1-q}$, so that $c = \psi_q(\beta) \cdot \pi_0 (\textcolor{red}{\vz})^{1-q}$
% % % \begin{align*}
% % %     \pi_{t,q}(\z) &=  \exp_q \left\{ (1-\beta_t) \ln_q \pi_0(\z) + \beta_t \ln_q \pi_1(\z)  - \psi_q \cdot \pi_0(\z)^{1-q} \right\} \\
% % %     ...\\
% % %     &= \left[ 1 + (1-q) \left( \ln_q \pi_0(\z) + t \left( \ln_q \pi_1(\z) - \ln_q \pi_0(\z) \right)\right)- (1-q) \psi_q \cdot \pi_0(\z)^{1-q} \right]_{+}^{\frac{1}{1-q}} \\
% % %     &= \left[ 1 + (1-q) \frac{1}{1-q} \left( \pi_0(\z)^{1-q} - 1  + t \big( \pi_1(\z)^{1-q} - 1 - \pi_0(\z)^{1-q} + 1 \big)\right) - (1-q) \psi_q \cdot \pi_0(\z)^{1-q}   \right]_{+}^{\frac{1}{1-q}} \\
% % %   &= \left[ 1 +  \pi_0(\z)^{1-q} - 1  + t \bigg( \pi_1(\z)^{1-q}  - \pi_0(\z)^{1-q} \bigg)  - (1-q) \psi_q \cdot \pi_0(\z)^{1-q}  \right]_{+}^{\frac{1}{1-q}} \\
% % %   &= \left[  \pi_0(\z)^{1-q}  + t \, \pi_1(\z)^{1-q} - t \, \pi_0(\z)^{1-q}   - (1-q) \psi_q \cdot \pi_0(\z)^{1-q} \right]_{+}^{\frac{1}{1-q}} \\
% % %     &= \left[  \pi_0(\z)^{1-q} \left(1 +  t \, \bigg(\frac{\pi_1(\z)}{\pi_0(\z)}\bigg)^{1-q} - t - (1-q) \psi_q \right)    \right]_{+}^{\frac{1}{1-q}} \\
% % %     &= \pi_0(\z) \left[ 1 +  (1-q)  \cdot \left( t \cdot \ln_q \frac{\pi_1(\z)}{\pi_0(\z)}  - \psi_q \right) \right]_{+}^{\frac{1}{1-q}} \\
% % %     &= \pi_0(z) \, \exp_q \big\{ \beta_ t \cdot \ln_q \frac{\pi_1(\z)}{\pi_0(\z)} - \psi_q  \big\}
% % % \end{align*}
% % % \text{ which matches \eqref{eq:lnq_fam}.}
% % %\end{proof}

% % \section{\texorpdfstring{$\alpha$}{}-Integration}\label{app:alpha_integration}
% % \citet{amari2007integration} show that the $\alpha$-mixture $\pi_{\alpha_t}$ minimizes the expected divergence to a single point.
% % \begin{align}
% % \pi_{\alpha_t}(\vz) &= \argmin \limits_{r(\vz)} \sum \limits_{i=1}^{N} w_i \, D_{\alpha}[p_i (\vz) : r(\vz) ] \label{eq:amari_vrep} \\
% % \text{where} \quad \pi_{\alpha_t}(\vz) &= \big( \sum \limits_{i=1}^{N} w_i \, p_i (\vz)^{\frac{1-\alpha}{2}}     \big)^{\frac{2}{1-\alpha}} \label{eq:alpha_mix_app}
% % \end{align}
% % \begin{proof}
% % \begin{align}
% % \frac{d}{dr} \sum \limits_{i=1}^{N} w_i \, D_{\alpha}[p_i (\vz) : r(\vz) ] &= \frac{d}{dr} \frac{4}{1-\alpha^2} \sum \limits_{i=1}^{N} w_i \big( -\int p_i(\vz)^{\frac{1-\alpha}{2}}\, r(\vz)^{\frac{1+\alpha}{2}} d\vz  +  \frac{1+\alpha}{2} \int r(\vz) d\vz \big) \\
% % 0 &=\frac{4}{1-\alpha^2} \big( -{\frac{1+\alpha}{2}} \sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}}\, r(\vz)^{\frac{1+\alpha}{2}-1} + \frac{1+\alpha}{2} \big) \\
% % - \frac{2}{1-\alpha} &= -\frac{2}{1-\alpha} \sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}}  r(\vz)^{-\frac{1-\alpha}{2}} \\
% %  r(\vz)^{\frac{1-\alpha}{2}} &= \sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}} \\
% %   r(\vz) &= \bigg(\sum \limits_{i=1}^{N} w_i  \, p_i(\vz)^{\frac{1-\alpha}{2}} \bigg)^{\frac{2}{1-\alpha}}
% % \end{align}
% % \end{proof}
% % %The function $f_{\alpha}(p) = \frac{2}{1-\alpha} \, p^{\frac{1-\alpha}{2}}$ is known as the $\alpha$-representation of a distribution $p$ \cite{amari2016information}.
% % This result is similar to a general result about Bregman divergences in \citet{Banerjee2005} Prop. 1, although $D_{\alpha}$ is not a Bregman divergence.

% % \subsection{Arithmetic Mean ($\alpha = -1$)}\label{app:mixture_path}
% % \newcommand{\pa}{\pi_0}%{p_a}
% % \newcommand{\pb}{\pi_1}%{p_b}
% % \newcommand{\opt}{r}%{q}
% % %\section{Relationship between \texorpdfstring{$\alpha$}{}-mean path and Grosse's moment averaging path}\label{app:grosse_alpha}
% % The moment-averaging path from \citet{grosse2013annealing} is \textit{not} a special case of the $\alpha$-mean path of \citet{amari2007integration}.   While both minimize a convex combination of reverse \textsc{kl} divergences, \citet{grosse2013annealing} minimize within the constrained space of exponential families %\textit{minimal exponential families}
% % , while \citet{amari2007integration} optimizes over \textit{all} normalized distributions.

% % More formally, consider minimizing the functional
% % \begin{align}
% %     J[\opt] &= (1 - \beta)\int \pa(z) \log \frac{\pa(z)}{\opt(z)} dz + \beta \int \pb(z) \log \frac{\pb(z)}{\opt(z)} dz \\
% %          &= \text{const} - \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \log \opt(z) dz \label{eq:functional}
% % \end{align}
% % We will show how \citet{grosse2013annealing} and \citet{amari2007integration} minimize \eqref{eq:functional}.



% % %\paragraph{Grosse's solution}
% % \paragraph{Solution within Exponential Family}
% % \citet{grosse2013annealing} constrains $\opt(z) = \frac{1}{Z(\theta)} h(z) \exp (\theta^T g(z))$ to be a (minimal) exponential family model and minimizes \ref{eq:functional} w.r.t $\opt$'s  natural parameters $\theta$ (cf. \cite{grosse2013annealing} appendix 2.2):
% % \begin{align}
% %     \theta^*_i &= \argmin_\theta J(\theta) \\
% %     &= \argmin_\theta \left(- \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \left[ \log h(z) + \theta^T g(z) - \log Z(\theta) \right] dz \right)\\
% %     &= \argmin_\theta \left(\log Z(\theta) - \int \left[(1 - \beta) \pa(z) + \beta \pb(z) \right] \theta^T g(z) dz  + \text{const}\right)
% % \end{align}
% % where the last line follows because $\pa(z)$ and $\pb(z)$ are assumed to be correctly normalized. Then to arrive at the moment averaging path, we compute the partials $\frac{\partial J(\theta)}{\partial \theta_i}$ and set to zero:
% % \begin{align}
% %     \frac{\partial J(\theta)}{\partial \theta_i} &= \E_{\opt}[g_i(z)] - (1 - \beta)\E_{\pa}[g_i(z)] - \beta \E_{\pb}[g_i(z)] = 0 \\
% %     \E_{\opt}[g_i(z)] &= (1 - \beta)\E_{\pa}[g_i(z)] - \beta \E_{\pb}[g_i(z)]
% % \end{align}
% % where we have used the exponential family identity $\frac{\partial \log Z(\theta)}{\partial \theta_i} = \E_{\opt_{\theta}}[g_i(z)]$ in the first line.



% % \paragraph{General Solution}
% % %\paragraph{Amari's solution}
% % Instead of optimizing in the space of minimal exponential families, \citet{amari2007integration} instead adds a Lagrange multiplier to \eqref{eq:functional} and optimizes $\opt$ directly (cf. \cite{amari2007integration} eq. 5.1 - 5.12)
% % \begin{align}
% %     {\opt}^* &= \argmin_{\opt} J'[\opt] \\
% %     &= \argmin_{\opt} J[\opt] + \lambda \left(1 - \int \opt(z) dz\right) \label{eq:lagrange}
% % \end{align}
% % \ref{eq:lagrange} can be minimized using the Euler-Lagrange equations or using the identity
% % \begin{align}
% %     \frac{\delta f(x)}{\delta f(x')} = \delta(x - x')\label{eq:delta_eq}
% % \end{align}
% % from \cite{meng2004introduction}. We compute the functional derivative of $J'[\opt]$ using \ref{eq:delta_eq} and solve for $q$:
% % \begin{align}
% %     \frac{\delta J'[\opt]}{\delta \opt(z)}=&- \int \big[(1 - \beta) \pa(z') + \beta \pb(z') \big] \frac{1}{\opt(z')} \frac{\delta \opt(z')}{\delta \opt(z)} dz' - \lambda \int \frac{\delta \opt(z')}{\delta \opt(z)} dz' \\
% %     =&- \int \big[(1 - \beta) \pa(z') + \beta \pb(z') \big] \frac{1}{\opt(z')} \delta(z - z') dz' - \lambda \int \delta(z - z') dz' \\
% %     =&- \big[(1 - \beta)\pa(z) + \beta \pb(z)\big] \frac{1}{\opt(z)} - \lambda = 0
% % \end{align}
% % Therefore
% % \begin{align}
% %     \opt(z) \propto \big[(1 - \beta)\pa(z) + \beta \pb(z)\big],
% % \end{align}
% % which corresponds to our $q$-path at $q=0$, or $\alpha = -1$ in \citet{amari2007integration}.  Thus, while both \citet{amari2007integration} and \citet{grosse2013annealing} start with the same objective, they arrive at different optimum because they optimize over different spaces.






==> sections/app/old/breg_table.tex <==
\section{Comparison of Exponential Family and $q$-Exponential Family}\label{app:breg_table}
\begin{table}[h]
\centering
\caption{\label{tab:properties}}
\begin{tabular}{p{2cm} p{6.1cm} p{6.5cm}} % \cmidrule(r){1-1}
  \cmidrule(lr){2-2} \cmidrule(l){3-3} \\[.25ex]
 & Exponential Family ($q=1$) & $q$-Exponential Family \\ \midrule
Definition & $\pi_{\beta}(\z) = \pi_0(\z) \, \exp \{ \beta \cdot \phi(\z) - \psi(\beta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z) \, \exp_q \{ \lambda \cdot \phi(\z) - \psi_q(\lambda) \} $ \\[2ex]
Free Energy & $\psi(\beta)  = \ln Z_{\beta} $ & $\psi_q(\lambda)$ \\[2ex]
Escort Dist. & $\Pi_{\beta, 1} =  \pi_0(\z)^{1-1} \, \pi_{\beta}(\z)^1 =  \pi_{\beta}(\z)  $ & $ \Pi_{\lambda,q} = \dfrac{1}{z_{q}(\lambda)} \pi_0(\z)^{1-q} \, \pi_{\lambda,q}(\z)^q $ \\[2ex]
Dual Params 		& $\dfrac{\partial \psi(\beta)}{\partial \beta^j} = \eta^j =  \mathbb{E}_{\pi_{\beta}}[\phi_j(\z)]$    \, (standard)		& $\dfrac{\partial \psi_q(\lambda)}{\partial \lambda^j} =\eta^j_q =\mathbb{E}_{\Pi_{\lambda,q}}[\phi_j(\z)] $ \, (escort) \\[2ex]
Bregman Div. & $D_{\psi}[\beta^{\prime} : \beta ] = D_{KL}[ \pi_{\beta} || \pi_{\beta^{\prime}} ] $ & $D_{\psi_q}[\lambda^{\prime} : \lambda ] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda,q}}{\pi_0} - \ln_q \dfrac{\pi_{\lambda^{\prime},q}}{\pi_0}] $ \\[2ex]
& $\phantom{D_{\psi}[\beta^{\prime} : \beta ]} = \mathbb{E}_{\pi_{\beta}} [ \ln \pi_{\beta} - \ln \pi_{\beta^{\prime}} ]$ &  \\[2ex]
Conjugate $\psi^{*}$ & $\psi^{*}(\eta) = D_{\psi}[\pi_0 ||  \pi_{\beta_{\eta}}] =D_{KL}[\pi_{\beta_{\eta}}||\pi_0 ] $ & $\psi_q^{*}(\eta) = D_{\psi_q}[\pi_0 ||\pi_{\lambda_{\eta},q}] = \mathbb{E}_{\Pi_{\lambda, q} }[ \ln_q \dfrac{\pi_{\lambda_{\eta},q}}{\pi_0} ] $\\[2ex] 
& & $\phantom{\psi_q^{*}(\eta) = } \hfill = \dfrac{1}{1-q}\bigg(\dfrac{1}{z_q(\lambda)} -1 \bigg) $ \\[3.5ex] \\
Neg. Entropy & $\psi^{*}(\eta) = \mathbb{E}_{\pi_{\beta_{\eta}}}[ \log \pi_{\beta_{\eta}} ] $\footnotesize \quad (if $\pi_0 =$uniform)& $\psi_q^{*}(\eta) = \mathbb{E}_{\Pi_{\lambda, q}}[ \ln_q \pi_{\lambda_{\eta},q} ] $  \footnotesize \quad (if $\pi_0 = $uniform) \\[3ex]
\small Dual Definition & $\pi_{\beta}(\z) = \pi_0(\z) \exp \{ \beta \, ( \phi(\z) - \eta ) + \psi^{*}(\eta) \}$  & $\pi_{\lambda}(\z) = \pi_0(\z)\exp_q \{ \lambda \, ( \phi(\z) - \eta_q ) + \psi_q(\lambda) \}$ \\
\bottomrule
\end{tabular}
\end{table}


==> sections/app/old/geo.tex <==
\newcommand{\alphaainv}{{\frac{2}{1-\alpha}}}
\newcommand{\alphaa}{{\frac{1-\alpha}{2}}}
\newcommand{\alphaaneg}{{\frac{1+\alpha}{2}}}
\newcommand{\alphaaneginv}{{\frac{2}{1+\alpha}}}

\section{\citet{zhang2013nonparametric} Geodesics }
This section closely follows \citet{zhang2013nonparametric} Sec. 2.2-2.3.
We will seek to show that our $q$-path
\begin{align}
    \ln_q \big(\tpi_{t, q}(z)\big) = (1-t) \ln_q \big(\tpi_{0}(z)\big) + t \, \ln_q \big(\tpi_{1}(z) \big)
\end{align}
forms a geodesic for the affine connection induced by the $\alpha$-divergence $D_{\alpha}$ over unnormalized measures.


Consider the $\rho, \tau$ embeddings
\begin{align}
    \rho(\tpi(z)) =  \alphaainv \big( \tpi(z)^\alphaa - 1 \big) \qquad \tau(\tpi) = \alphaaneginv  \big( \tpi(z)^\alphaaneg - 1 \big)
\end{align}
which are conjugate with respect to the function
\begin{align}
    f(\rho) = \alphaaneginv \big( 1 + \alphaa \cdot \rho)^\alphaainv
\end{align}
where conjugacy means that $\tau(\tpi(z)) = f^{\prime}\big(\rho(\tpi(z))\big)$.


This induces a family of $\alpha$-divergences $D^{(\alpha)}_{f,\rho}$, where $\alpha$ is intended to reflect \textit{referential duality}.   Our use of $\alpha$ in the $\rho, \tau$ embedding functions, or $q$ in the $\ln_q$ path, rather reflects \textit{representational duality} in terms of the $\alpha$-representation (e.g. \citet{amari2010divergencefunctions}).

% geodesic is wrt second argument
We obtain the flat divergence, which integrates an expression of Bregman form
\begin{align}
    D^{(1)}_{f, \rho}[\tpi_a:\tpi_b] =  \int f\big(\rho(\tpi_a(z)) \big) -  f\big(\rho(\tpi_b(z)) \big) + \big( \rho(\tpi_a(z)) - \rho(\tpi_b(z)) \big) \cdot  \tau(\tpi_b) dz
\end{align}
which can be shown to correspond to Amari's $\alpha$ divergence for the choice of $f, \rho$ above.
\begin{align}
D^{(1)}_{f, \rho}[\tpi_a:\tpi_b] &= D_{\alpha}[\tpi_a(\vz):\tpi_b(\vz) ] \\
&= \frac{4}{(1-\alpha^2)} \bigg( \frac{1-\alpha}{2}  \int \tpi_a(\vz) \,d\vz +  \frac{1+\alpha}{2}  \int \tpi_b(\vz) \,d\vz -\int \tpi_a(\vz)^{\frac{1-\alpha}{2}} \, \tpi_b(\vz)^{\frac{1+\alpha}{2}}  d\vz  \bigg)
\end{align}
As shown in Proposition 2 and Corollary 3 of \citet{zhang2013nonparametric}, we can define an information manifold $(\mathcal{M}_+, g_{ij}^{(D^{(1)}_{f,\rho})}, \nabla^{(1)}, \nabla^{(-1)})$.   See \citet{zhang2013nonparametric} for additional details.   We consider only the affine connection $\nabla^{(1)}$ in what follows, which is a special case of the $\alpha$-connection for the above manifold
\begin{align*}
    \nabla^{(\alpha)}_{\dot{\gamma}} \dot{\gamma} = (d_{\dot{\gamma}} \dot{\gamma})_{\gamma_t} + \frac{d}{d\gamma} \big( \alphaaneg \log \rho^{\prime}(\gamma(t)) + \alphaa \log \tau^{\prime}(\gamma(t)) \big) \label{eq:affine_alpha}
\end{align*}



\subsection{$q$-Path as Geodesic}
Our $q$-path distributions $\tpi_{t, q}$ along a curve parameterized by $t$, are defined using the power mean with function $\rho(u)$, and are thus linear in the $\rho$ representation
\begin{align}
    \rho\big( \gamma(t)\big) = \rho\big(\tpi_{t, q}(z)\big) = (1-t) \rho\big(\tpi_{0}(z)\big) + t \, \rho\big(\tpi_{1}(z) \big)
\end{align}
where $\rho(u) = \ln_q(u)$ for $q = 2\alpha-1$. %(see Eq. \eqref{eq:lnqexpq}).

We seek to show that our $q$-path is a geodesic with respect to the affine connection $\nabla^{(1)}$, or an autoparallel path.  Let $\gamma_t = \gamma(t) = \tpi_{t,q}(z)$ indicate the $q$-path distribution with mixing parameter $t$, with $\dot{\gamma} = d \gamma_t / dt$.

Plugging $\alpha = 1$ into \eqref{eq:affine_alpha} , and with $ (d_{\dot{\gamma}} \dot{\gamma})_{\gamma_t} = \frac{d \dot{\gamma(t)}}{d\gamma_t} \cdot \dot{\gamma}$ , we seek to show that $\nabla_{\dot{\gamma}} \dot{\gamma} = 0$, or
\begin{align*}
    \nabla^{(1)}_{\dot{\gamma}} \dot{\gamma} = \frac{d \dot{\gamma}}{d\gamma} \cdot \dot{\gamma} + \big(\dot{\gamma}\big)^{2} \cdot \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big)
\end{align}


We will first derive several useful quantities.  Since it is easier to differentiate $\rho(\gamma(t)) = (1-t) \rho(\pi_0) + t \, \rho(\tpi_1)$ with respect to $\gamma$, we note that $\frac{d}{dt} \rho\big( \gamma(t) \big) = \frac{d \rho(\gamma) }{d\gamma(t)} \frac{d\gamma(t)}{dt}$.  We can then rewrite the desired $\frac{d\gamma(t)}{dt}$ as
\begin{align}
    \dot{\gamma} = \frac{d\gamma(t)}{dt} &= \bigg( \frac{d \rho(\gamma_t) }{d\gamma(t)} \bigg)^{-1} \, \frac{d \rho(\gamma_t) }{dt} = \gamma^{\alphaaneg} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \\[1.4ex]
    \implies  \dot{\gamma} &=\gamma_t \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \quad (\text{for $\alpha = 1$}) \label{eq:dgamma_dt}
\end{align}
since
\begin{align}
    \frac{d \rho(\gamma_t) }{d\gamma_t}  &= \frac{d}{d \gamma_t} \alphaainv \big( \gamma^\alphaa - 1 \big) = \gamma_t^{\alphaa - \frac{2}{2}} =  \gamma_t^{\frac{-(1+\alpha)}{2}} \\
    \text{and } \quad \frac{d \rho(\gamma_t) }{dt}  &= \frac{d}{dt} \big( (1-t) \rho(\pi_0) + t \, \rho(\tpi_1) \big) = \rho(\tpi_1) - \rho(\pi_0)
\end{align}

We can now differentiate the $\frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) $ term in the affine connection.   From above, $d \rho(\gamma_t) / d\gamma(t) = \gamma_t^{\frac{-(1+\alpha)}{2}}$, so that
\begin{align}
    \frac{d}{d\gamma} \big(  \log \frac{d}{d\gamma} \rho(\gamma(t)) \big) &=   \frac{d}{d\gamma}   \log \big( \gamma_t^{\frac{-(1+\alpha)}{2}} \big) = -\frac{(1+\alpha)}{2} \cdot \frac{d}{d\gamma}   \log \gamma_t \\
    &\phantom{\frac{d}{d\gamma}   \log \big( \gamma_t^{\frac{-(1+\alpha)}{2}} \big)} = -\frac{(1+\alpha)}{2} \gamma_t^{-1} \\
    % &= \gamma_t^{\frac{(1+\alpha)}{2}} \cdot \frac{d}{d\gamma} \gamma_t^{\frac{(1+\alpha)}{2}} \\
    % % &=
    % % \bigg( \frac{d}{d\gamma} \rho(\gamma_t) \bigg)^{-1} \cdot \frac{d}{d\gamma}  \rho(\gamma_t) \\
    % &= \gamma^{\frac{(1+\alpha)}{2}} \cdot  - \frac{(1+\alpha)}{2} \gamma^{-\frac{(1+\alpha)}{2}-1} \\
    % &= -\gamma_t \cdot \gamma_t^{-2} \\
    \implies \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) &=  -\gamma_t^{-1} \quad (\text{for $\alpha=1$}) \label{eq:db_dgamma}
\end{align}


Putting it all together, and with dot products turning into scalar products for our one-dimensional curve $t$, we have
\begin{align}
    \nabla^{(1)}_{\dot{\gamma}} \dot{\gamma} &=  \frac{d \dot{\gamma}}{d\gamma_t} \cdot \dot{\gamma}  + \big(\dot{\gamma}\big)^{2} \frac{d}{d\gamma} \big(  \log \rho^{\prime}(\gamma(t)) \big) \\
    &=  \frac{d }{d\gamma_t} \bigg( \gamma_t \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \bigg) \cdot \dot{\gamma}  -  (\dot{\gamma})^{2} \gamma_t^{-1}
    \qquad \quad \text{(using \eqref{eq:dgamma_dt} and \eqref{eq:db_dgamma})} \\
    &= \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) - (\dot{\gamma})^{2} \cdot {\dot{\gamma}}^{-1} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \qquad \text{(rearranging \eqref{eq:dgamma_dt})} \\
    &= \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) - \dot{\gamma} \cdot \big( \rho(\tpi_1) - \rho(\pi_0) \big) \\
    &=0
\end{align}

\clearpage
\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_09.pdf}}
    \subfigure[$q=0.9$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_18.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/figs/gif/ridge_20.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_12_redo.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_2_redo.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_3_redo.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_4_redo.pdf}}
    \caption{Intermediate densities between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$ for various $q$-paths and 10 equally spaced $\beta$. The path approaches a mixture of Gaussians with  weight $\beta$ at $q=0$.  For the geometric mixture ($q=1$), intermediate $\pi_{\beta}$ stay within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:alpha_path}
    \vspace*{-.15cm}
\end{figure}


\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha-1_student_df2_2.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha05_student_df2_2.pdf}}
    \subfigure[$q=0.95$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha95_student_df2_2.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha1_student_df2_2.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha11_student_df2_2.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha15_student_df2_2.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha2_student_df2_2.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha3_student_df2_2.pdf}}
    \caption{Intermediate densities between $\text{Student}(\text{df}=2, -4, 3)$ and $\text{Student}(\text{df}=2, 4, 1)$ for various $q$-paths and 10 equally spaced $\beta$.}
    \label{fig:q_path}
    \vspace*{-.15cm}
\end{figure}



\begin{figure}[t]
    \centering
    \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha-1_student_df2_2.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha05_student_df2_2.pdf}}
    \subfigure[$q=0.95$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha95_student_df2_2.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.24\textwidth]{sections/app/draft_figs/ridge_alpha1_student_df2_2.pdf}}
    \subfigure[$q=1.1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha11_student_df2_2.pdf}}
    \subfigure[$q=1.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha15_student_df2_2.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha2_student_df2_2.pdf}}%
    \subfigure[$q=3$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.23\textwidth]{sections/app/draft_figs/ridge_alpha3_student_df2_2.pdf}}
    \caption{Tail behavior for densities between $\text{Student}(\text{df}=2, -4, 3)$ and $\text{Student}(\text{df}=2, 4, 1)$ for various $q$-paths and 10 equally spaced $\beta$.}
    \label{fig:q_path}
    \vspace*{-.15cm}
\end{figure}


==> sections/app/old/student.tex <==
\newcommand{\qqq}{{q}}
\newcommand{\qqexp}{{1-q}}
\newcommand{\qqexpconj}{{q}}
\newcommand{\qqinv}{{{\frac{1}{1-q}}}}
\newcommand{\bmu}{{\mathbf{\mu}}}
\newcommand{\bSig}{{\mathbf{\Sigma}}}

\section{Annealing between Student-$t$ Distributions}\label{app:additional}

% \paragraph{Discrete}
% Consider a finite sample space of $M$ events $\{x_1, ... x_M \}$, with sufficient statistics $\phi_i(\vx) = \delta_i(\vx) = \mathbb{I}(\vx = \vx_i)$ indicating whether the observation $\vx$ matches event $\vx_i$.   We can define each element of the parameter vector $\theta = \{ \theta_1, ... \theta_M \}$ as a difference of $\ln_\qqq$ probabilities, where the final index $\ln_\qqq p(\vx_M)$ enforces normalization.
% \begin{align}
%     \theta_i = \ln_\qqq p(\vx_i) - & \ln_\qqq p(\vx_M) \qquad \psi_\qqq(\theta) = -\ln_\qqq p(\vx_M) \\
%     \pi_\theta(\vx_i) &= \exp_\qqq \{ \theta \cdot \phi(\vx) - \psi(\theta) \} \\
%     &= \exp_\qqq \{ \ln_\qqq p(\vx_i) - \ln_\qqq p(\vx_M) + \ln_\qqq p(\vx_M) \} \\
%     &= p(\vx_i)
% \end{align}
% Thus, for any order $\qqq$, a discrete distribution is a $\qqq$-exponential family.

\subsection{Student-$t$ Distributions and $q$-Exponential Family}
The Student-$t$ distribution appears in hypothesis testing with finite samples, under the assumption that the sample mean follows a Gaussian distribution.   In particular, the degrees of freedom parameter $\nu = n-1$ can be shown to correspond to an order of the $\qqq$-exponential family with $\nu = (3-\qqq) / (\qqq-1)$ (in 1-d), so that the choice of $\qqq$ is linked to the amount of data observed.

We can first write the multivariate Student-$t$ density, specified by a mean vector $\mu$, covariance $\bSig$, and degrees of freedom parameter $\nu$, in $d$ dimensions, as
\begin{align}
    t_{\nu}(\vx | \bmu, \bSig) = \frac{1}{Z(\nu, \bSig)} \big[ 1 + \frac{1}{\nu} (x - \bmu)^T \bSig^{-1} (x-\bmu) \big]^{-\big(\frac{\nu + d }{2}\big)} \label{eq:student}
\end{align}
where $Z(\nu, \bSig) = \Gamma(\frac{\nu+d}{2})/\Gamma(\frac{\nu}{2}) \cdot |\bSig|^{-1/2} \nu^{-\frac{d}{2}} \pi^{-\frac{d}{2}}$.  Note that  $\nu > 0$, so that we only have positive values raised to the $-(\nu+d)/2$ power, and the density is defined on the real line.

The power function in \eqref{eq:student} is already reminiscent of the $\qqq$-exponential, while we have first and second moment sufficient statistics as in the Gaussian case.  We can solve for the exponent, or order parameter $q$, that corresponds to $-(\nu+d)/2$ using $-\big(\frac{\nu + d }{2}\big) = \frac{1}{1-\qqq}$.  This results in the relations
\begin{align}
 \nu = \frac{d - d \qqq +2}{\qqq - 1} \qquad \text{or} \qquad \qqq = \frac{\nu+d+2}{\nu+d}
\end{align}
We can also rewrite the $\nu^{-1} \, (x - \bmu)^T \bSig^{-1} (x-\bmu) $ using natural parameters corresponding to $\{x, x^2\}$ sufficient statistics as in the Gaussian case (see, e.g. \citet{matsuzoe2015deformed} Example 4).

Note that the Student-$t$ distribution has heavier tails than a standard Gaussian, and reduces to a multivariate Gaussian as $\qqq \rightarrow 1$ and $\exp_{\qqq}(u) \rightarrow \exp(u)$.  This corresponds to observing $n\rightarrow \infty$ samples, so that the sample mean and variance approach the ground truth \cite{murphy2007conjugate}. %, which was assumed to follow a Gaussian distribution,

\begin{figure}[t]
    \centering
    \subfigure[$q=0$] {\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_09.pdf}}
    \subfigure[$q=0.9$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.2\textwidth]{sections/figs/gif/ridge_18.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_20.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 .1cm 0.25cm 0 },clip,width=0.19\textwidth]{sections/figs/gif/gaussian_2.pdf}}
    \caption{Intermediate densities between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$ for various $q$-paths and 10 equally spaced $\beta$. The path approaches a mixture of Gaussians with  weight $\beta$ at $q=0$.  For the geometric mixture ($q=1$), intermediate $\pi_{\beta}$ stay within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:alpha_path22} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.
    %\caption{Intermediate densities using various $q$-paths between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$, with 10 equally spaced $\beta$. The $q$-path approaches a mixture of Gaussians with mixing parameter $\beta$ at $q=0$.  For the geometric mixture at $q=1$, the path remains within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:gaussian_path} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.\
    \vspace*{-.15cm}
\end{figure}%
\begin{figure}[t]
    \centering
    % \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \includegraphics[trim={0 0 0 0 },clip,width=0.99\textwidth]{sections/figs/student_t.pdf}
    \caption{Intermediate densities between Student-$t$ distributions, $t_{\nu = 1}(-4, 3)$ and $t_{\nu = 1}(4,1)$ for various $q$-paths and 10 equally spaced $\beta$,
    Note that $\nu=1$ corresponds to $q=2$, so that the $q=2$ path stays within the $q$-exponential family.\\[3ex]
    We provide code to reproduce experiments at \url{https://github.com/vmasrani/q\_paths}.
    }
    \label{fig:alpha_path} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.
    %\caption{Intermediate densities using various $q$-paths between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$, with 10 equally spaced $\beta$. The $q$-path approaches a mixture of Gaussians with mixing parameter $\beta$ at $q=0$.  For the geometric mixture at $q=1$, the path remains within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:student_path} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.\
    \vspace*{-.15cm}
\end{figure}

\subsection{Annealing between 1-d Student-$t$ Distributions}
Since the Student-$t$ family generalizes the Gaussian distribution to $q \neq 1$, we can run a similar experiment annealing between two Student-$t$ distributions.   We set $q=2$, which corresponds to $\nu = 1$ with $\nu = (3-\qqq) / (\qqq-1)$, and use the same mean and variance as the Gaussian example in Fig. \ref{fig:alpha_path22}, with $\pi_0(z) = t_{\nu=1}( -4, 3)$ and $\pi_1(z) = t_{\nu=1}( 4, 1)$.

We visualize the results in Fig. \ref{fig:student_path}.   For this special case of both endpoint distributions within a parametric family, we can ensure that the $q=2$ path stays within the $q$-exponential family of Student-$t$ distributions.   We make a similar observation for the Gaussian case and $q=1$ in Fig. \ref{fig:gaussian_path}.   Comparing the $q=0.5$ and $q=0.9$ Gaussian path with the $q=1.0$ and $q=1.5$ path, we observe that mixing behavior appears to depend on the relation between the $q$-path parameter and the order of the $q$-exponential family of the endpoints.

As $q \rightarrow \infty$, the power mean \eqref{eq:abstract_mean} approaches the $\min$ operation as $1-q \rightarrow -\infty$.    In the Gaussian case, we see that, even at $q=2$, intermediate densities for all $\beta$ appear to concentrate in regions of low density under both $\pi_0$ and $\pi_T$.   However, for the heavier-tailed Student-$t$ distributions, we must raise the $q$-path parameter significantly to observe similar behavior.

\newcommand{\base}{g}
\subsection{Endpoints within a Parametric Family}
If the two endpoints $\pi_0, \tpi_1$ are within a $q$-exponential family, we can show that each intermediate distribution along the $q$-path of the same order is also within this $q$-family.  However, we cannot make such statements for general endpoint distributions or members of  different $q$-exponential families.

\paragraph{Exponential Family Case}
We assume potentially vector valued parameters $\theta = \{ \theta\}_{i=1}^N$ with multiple sufficient statistics $\phi(\vz) = \{ \phi_i(\vz) \}_{i=1}^N$, with $\theta \cdot \phi(\vz) = \sum_{i=1}^N \theta_i \phi_i(\vz)$.
For a common base measure $\base(\vz)$, let $\pi_0(\vz) = \base(\vz) \, \exp\{ \theta_0 \cdot \phi(\vz) \}$ and $\tpi_1(\vz) = \base(\vz) \, \exp \{ \theta_1 \cdot \phi(\vz) \}$.   Taking the geometric mixture,
\begin{align}
    \tpi_\beta(\vz) &= \exp \big\{ (1-\beta) \, \log \pi_0(\vz) + \beta \, \log \tpi_1(\vz) \big\} \\
    &= \exp \big \{ \log \base(\vz) + (1-\beta) \, \theta_0 \cdot \phi(\vz) + \beta  \, \theta_1 \phi(\vz)  \big \} \\
    &= \base(\vz) \exp  \big \{ \big( (1-\beta) \, \theta_0 + \beta  \, \theta_1 \big) \cdot \phi(\vz)  \big \}
\end{align}
which, after normalization, will be a member of the exponential family with natural parameter $(1-\beta) \, \theta_0 + \beta  \, \theta_1$.




\paragraph{$q$-Exponential Family Case} For a common base measure $\base(\vz)$, let $\pi_0(\vz) = \base(\vz) \, \exp_q \{ \theta_0 \cdot \phi(\vz) \}$ and $\tpi_1(\vz) = \base(\vz) \, \exp_q \{ \theta_1 \cdot \phi(\vz) \}$.   The $q$-path intermediate density becomes
\begin{align}
\tilde{\pi}^{(q)}_\beta(\vz) &= \big[ (1-\beta) \, \pi_0(\vz)^{1-q} + \beta \, \tpi_1(\vz)^{1-q} \big]^{\frac{1}{1-q}} \\
&= \big[ (1-\beta) \, \base(\vz)^{1-q} \, \exp_q \{ \theta_0 \cdot \phi(\vz) \}^{1-q} + \beta \, \base(\vz)^{1-q} \,\exp_q \{ \theta_1 \cdot \phi(\vz) \} ^{1-q} \big]^{\frac{1}{1-q}} \\
&=  \bigg[ \base(\vz)^{1-q} \bigg ( (1-\beta) \,  \, [1 + (1-q)( \theta_0 \cdot \phi(\vz))]^{\frac{1}{1-q}1-q} + \beta  \, [1 + (1-q)( \theta_1 \cdot \phi(\vz))]^{\frac{1}{1-q} 1-q} \bigg) \bigg]^{\frac{1}{1-q}} \nonumber \\
&= \base(\vz) \bigg[ 1 + (1-q) \bigg( \big((1-\beta) \, \theta_0 + \beta  \, \theta_1 \big)  \cdot \phi(\vz) \bigg) \bigg]^{\frac{1}{1-q}} \\
&= \base(\vz) \exp_q \big\{  \big((1-\beta) \, \theta_0 + \beta  \, \theta_1 \big) \cdot \phi(\vz) \big\}
\end{align}
which has the form of an unnormalized $q$-exponential family density with parameter $(1-\beta) \, \theta_0 + \beta  \, \theta_1$.
%\begin{align}
%     \tilde{\pi}^{(q)}_\beta(\vz) = \begin{cases}\big[ (1-\beta) \, \pi_0(\vz)^{1-q} + \beta \, \tpi_1(\vz)^{1-q} \big]^{\frac{1}{1-q}} & q \neq 1 \\[1.3ex]
%      \exp \big\{ (1-\beta) \, \log \pi_0(\vz) + \beta \, \log \tpi_1(\vz) \big\} & q = 1  \\[1.25ex]
%     \end{cases},  \label{eq:alpha_mix3}
% \end{align}



==> sections/app/old/vm_naudts_paths.tex <==
\section{Derivation of Path $q$-Family}\label{app:q_path}
With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
\begin{align}
    \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
\end{align}
which is suggestive of the convex conjugate for $\psi_q$ via
\begin{align}
    \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
\end{align}
We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

\begin{proof}
\begin{align}
    \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
    &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
\end{align}
Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
\begin{align}
    \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
    Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
\end{align}

To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
\begin{align}
    \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
\end{align}
and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
\begin{align}
    \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
    &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
\end{align}
where we have defined
\begin{align}
    \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
\end{align}
\end{proof}



\section{Alternative Derivation}
Note that $\exp_q \{ x + y \} = \exp_q \{ y \} \cdot \exp_q \{ \frac{x}{1 + (1-q) y}  \}$ from \textcolor{red}{Vaden's theorem below.}, instead of $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $ for the standard exponential.  This implies that
\begin{align}
\pi_{q,\beta} = \pi_0 \, \exp_q \{ \beta \cdot \phi(\vz) - \psi_q \} &= \pi_0 \, \exp_q\{ -\psi_q \} \exp_q \{ \frac{\beta}{1+(1-q)(-\psi_q)} \cdot \phi(\vz) \} 
\end{align}
Our goal is to express $\pi_{q,\beta}(\vz)$ using a normalization constant $Z$ instead of the $q$-free energy $\psi_q(\beta)$.  While the exponential family allows us to freely move between  $\log Z_{\beta}$
and $\psi(\beta)$, in the $q$-exponential case, we must adjust the parameters.   Defining
%To (w/ $\eta, \beta$ switched) match Naudts, let : }
\begin{align}
 \eta &= \frac{\beta}{1+(1-q)(-\psi_q)} \\
Z_q(\eta) &= \frac{1}{\exp_q \{-\psi_q \}} := \exp_{q}^{*}\{ -\psi_q\} \\
\end{align}
we obtain a new parameterization of the $q$-exponential family, using parameters $\eta$ and multiplicative normalization constant $Z_q(\eta)$, as
\begin{align}
 \pi_{q,\beta} =  \pi_{q,\eta} &=  \frac{1}{Z_q(\eta)} \exp_{q} \{ \eta \cdot \phi(\vz) \}
\end{align}
See \citet{matsuzoe2019normalization} for more detailed discussion of normalization in deformed exponential families.


==> sections/app/old/vm_q_sum_prod.tex <==
\section{Sum and Product Identities for $q$-Exponentials}\label{app:q_sum_product}
In this section, we prove two lemmas which are useful for manipulation expressions involving $q$-exponentials, for example in moving between \cref{eq:normalization1} and \cref{eq:normalization2} in either direction.
\begin{lemma}
    Sum identity
    \begin{align}
        \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
    \end{align}
    \label{lemma:q_exp_sum}
\end{lemma}
\begin{lemma}
    Product identity
    \begin{align}
        \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
    \end{align}
    \label{lemma:q_exp_prod}
\end{lemma}

\subsection{Proof of \cref{lemma:q_exp_sum}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
    \begin{align}
        \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \left[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \right]_{+}^{1/(1-q)} \\
                                                &= \left[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \right]_{+}^{1/(1-q)} \\
                                                &= \left[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \right]_{+}^{1/(1-q)} \\
                                                &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
                                                &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
    \end{align}
\end{proof}
\subsection{Proof of \cref{lemma:q_exp_prod}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + = (1 - q)x_i\right)$. Then, 
    %and $(1-q) = (1 - q)$. Then
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
    &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \hspace*{-.5cm} \text{(reindex $n \to n - 1)$} \nonumber \\
    &=\exp_q(x_{0})\exp_q(y_N) & \hspace*{-.5cm} \text{(inductive hypothesis)} \nonumber \\
    &= \bigg[\left(1 + (1-q) \cdot x_{0}\right)\left(1 + (1-q) \cdot y_N\right) \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \cdot x_{0} + \big(1 + (1-q) \cdot x_{0} \big)(1-q) \cdot y_N \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \bigg(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\bigg) \bigg]_{+}^{1/(1-q)}\\
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\right)
\end{align}
Next we use the definition of $y_N$ and rearrange
\begin{align}
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)\left(x_1 + x_2(1 + (1-q) \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + (1-q) \cdot x_i)\right)\right) \nonumber\\
    &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q) x_i\right)\right).
\end{align}
Then reindexing $n \to n + 1$ establishes
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q)x_i\right)\right).
\end{align}
\end{proof}


% \section{Sum Identity for $q$-exponentials}\label{app:q_sum_product}
% %\section{Sum and product identities for $q$-exponentials}\label{app:q_sum_product}
% While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $, this is not true for $\exp_{\alpha}\{ x + y \}$.   We derive a more general expression for the $q$-exponential below.
% %In the Lemma below, prove a more general statement for the $q$-exponential.
% %We therefore derive two lemmas for q-exponentials which will be useful in obtaining the $q$-exponential family. We will prove both statements by induction and simplify notation by defining $(1-q) := 1 - q$.

% \begin{lemma}
%     Sum identity
%     \begin{align}
%         \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
%         \begin{align}
%             \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \bigg]^{1/(1-q)} \\
%                                                     &= \bigg[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \bigg]^{1/(1-q)} \\
%                                                     &= \bigg[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \bigg]^{1/(1-q)} \\
%                                                     &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
%                                                     &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
%         \end{align}
%     \end{proof}
% \end{lemma}

% %\section{Sum and product identities for $q$-exponentials}\label{app:q_sum_product}
% While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $, this is not true for $\exp_{\alpha}\{ x + y \}$. We therefore derive two lemmas for q-exponentials which will be useful in obtaining the $q$-exponential family. We will prove both statements by induction and simplify notation by defining $\bar{q} := 1 - q$.

% \begin{lemma}
%     Sum identity
%     \begin{align}
%         \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$. Assuming \cref{eq:q_exp_sum} holds for $N$,
%         \begin{align}
%             \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + \bar{q} \sum_{n=1}^{N+1} x_n \bigg]^{1/\bar{q}} \\
%                                                     &= \bigg[ 1 + \bar{q} \left(\sum_{n=1}^{N} x_n\right) + \bar{q}x_{N+1} \bigg]^{1/\bar{q}} \\
%                                                     &= \bigg[\left( 1 + \bar{q} \sum_{n=1}^{N} x_n \right) \left(1 + \bar{q}\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n}\right) \bigg]^{1/\bar{q}} \\
%                                                     &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n} \right)\\
%                                                     &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + \bar{q}\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
%         \end{align}
%     \end{proof}
% \end{lemma}

% \begin{lemma}
%     Product identity
%     \begin{align}
%         \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)$. Then
%     \begin{align}
%         \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
%         &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \text{(reindex $n \to n - 1)$}\\
%         &=\exp_q(x_{0})\exp_q(y_N) & \text{(inductive hypothesis)}\\
%         &= \bigg[\left(1 + \bar{q} \cdot x_{0}\right)\left(1 + \bar{q} \cdot y_N\right) \bigg]^{1/\bar{q}}\\
%         &= \bigg[1 + \bar{q} \cdot x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\bar{q} \cdot y_N \bigg]^{1/\bar{q}}\\
%         &= \bigg[1 + \bar{q} \bigg(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\bigg) \bigg]^{1/\bar{q}}\\
%         &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\right)
%     \end{align}
%     Next we use the definition of $y_N$ and rearrange
%     \begin{align}
%         &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\left(x_1 + x_2(1 + \bar{q} \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + \bar{q} \cdot x_i)\right)\right)\\
%         &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q} x_i\right)\right).
%     \end{align}
%     Then reindexing $n \to n + 1$ establishes
%     \begin{align}
%         \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)\right).
%     \end{align}
% \end{proof}
% \end{lemma}







% \section{Derivation of Path $q$-Family}\label{app:q_path}
% \vm{This longer derivation is necessary to establish relationship between two q-exp fam forms and allow for tvo/ti trick. Might also be better to save for full paper and revert to prev}
% With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
% \begin{align}
%     \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
% \end{align}
% which is suggestive of the convex conjugate for $\psi_q$ via
% \begin{align}
%     \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
% \end{align}
% We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

% \begin{proof}
% \begin{align}
%     \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
%     &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
% \end{align}
% Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
% \begin{align}
%     \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
%     Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
% \end{align}

% To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
% \begin{align}
%     \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
% \end{align}
% and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
% \begin{align}
%     \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
%     &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
% \end{align}
% where we have defined
% \begin{align}
%     \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
% \end{align}
% \end{proof}


==> sections/app/student.tex <==
\section{Annealing between Student-$t$ Distributions}\label{app:additional}

\paragraph{Student-$t$ Distribution}
\vm{Moved from main}
The Student-$t$ distribution appears in hypothesis testing with finite samples, under the assumption that the sample mean follows a Gaussian distribution.   In particular, the degrees of freedom parameter $\nu = n-1$ can be shown to correspond to an order of the $q$-exponential family with $\nu = (3-q) / (q-1)$ (in 1-d), so that the choice of $q$ is linked to the amount of data observed.


We can first write the multivariate Student-$t$ density, specified by a mean vector $\mu$, covariance $\Sigma$, and degrees of freedom parameter $\nu$, in $d$ dimensions, as
\begin{align}
    t_{\nu}(\vx | \mu, \Sigma) = \frac{1}{Z(\nu, \Sigma)} \big[ 1 + \frac{1}{\nu} (x - \mu)^T \Sigma^{-1} (x-\mu) \big]^{-\big(\frac{\nu + d }{2}\big)} \label{eq:student}
\end{align}
where $Z(\nu, \Sigma) = \Gamma(\frac{\nu+d}{2})/\Gamma(\frac{\nu}{2}) \cdot |\Sigma|^{-1/2} \nu^{-\frac{d}{2}} \pi^{-\frac{d}{2}}$.  Note that  $\nu > 0$, so that we only have positive values raised to the $-(\nu+d)/2$ power, and the density is defined on the real line.

The power function in \eqref{eq:student} is already reminiscent of the $q$-exponential, while we have first and second moment sufficient statistics as in the Gaussian case.   Solving for the exponent, or order of $\exp_{q}$, that corresponds to $-(\nu+d)/2$, we obtain
\begin{align}
    -\big(\frac{\nu + d }{2}\big) = \frac{1}{1-q} \quad \implies \\
     q = \frac{\nu+d+2}{\nu+d} \quad \text{or} \quad \nu = \frac{d - d q +2}{q - 1}
\end{align}
We can also rewrite the $\nu^{-1} \, (x - \mu)^T \Sigma^{-1} (x-\mu) $ using natural parameters corresponding to $\{x, x^2\}$ sufficient statistics as in the Gaussian case (see, e.g. \citet{matsuzoe2015deformed} Example 4).

Note that the Student-$t$ distribution has heavier tails than a standard Gaussian, and reduces to a multivariate Gaussian as $q \rightarrow 1$ and $\exp_{q}(u) \rightarrow \exp(u)$.  This corresponds to observing $n\rightarrow \infty$ samples, so that the sample mean and variance approach the ground truth. %, which was assumed to follow a Gaussian distribution,

\citet{gelman2013bayesian} Sec. 3.3, 3.6
or \citet{murphy2007conjugate} Sec. 5,9 show that the Student-$t$ distribution with $\nu = n - d + 1$ degrees of freedom arises as the posterior predictive for either the unknown mean $\mu$ or a new data observation $x$, after observing $n$ samples from a $d$-dimensional Gaussian and assuming an inverse Wishart prior for the covariance.
\begin{align}
    p(\mu| x_{\leq n}, \kappa_n, \mu_n, S_n) = t_{\nu_n - d + 1} \big(\mu_n, \frac{S_n}{\kappa_n (\nu_n - d + 1) }\big)
\end{align}
where $\mu_n$ is the current estimate of the sample mean.  The predictive for an observation $x_{n+1}$ is similar, but with the variance scaled by $\frac{S_n \cdot (\kappa_n+1)}{\kappa_n (\nu_n - d + 1) }$.  Conjugate updates are easy for all parameters, with $\kappa_n$ and $\nu_n$ tracking the number of observations, $\mu_n$ and $S_n$ tracking the statistics from observed samples.

\paragraph{Pareto Distributions: Modeling Tail Events and Power Law Behavior}
The $q$-exponential family can also be used for modeling the \textit{tail} behavior of a distribution \citep{bercher2008new, bercher2008tsallis, vehtari2015pareto}, or, in other words, the probability of $p(x)$ restricted to $X > x_{\text{min}} $ and normalized.

For example, the generalized Pareto distribution is defined via the tail function
\begin{align}
    P(X > x) = \begin{cases}  \big(1 + \xi \frac{x-x_{\text{min}} }{\sigma} \big)^{-\frac{1}{\xi}} \quad \xi \neq 0 \\  \exp\{- \frac{x-x_{\text{min}} }{\sigma}\} \qquad \xi =0
    \end{cases}
\end{align}
When $\xi \geq 0$,  the domain is restricted to $x \geq x_{\text{min}}$, whereas when $\xi < 0$, the support is between $x_{\text{min}} \leq x \leq x_{\text{min}}-\frac{\sigma}{\xi}$. Writing the CDF as $1- P(X>x)$ and differentiating leads to
\begin{align}
    p(x) = \frac{1}{\sigma}\big[1 + \xi \cdot \frac{x-x_{\text{min}}}{\sigma}  \big]^{-\frac{1}{\xi}-1}
\end{align}
Solving $-\frac{1}{\xi}-1 = \frac{1}{1-q}$ in the exponent, we obtain $q = \frac{2\xi + 1}{\xi+1}$ or $\xi = \frac{q-1}{q-2}$ .



% \paragraph{Discrete}
% Consider a finite sample space of $M$ events $\{x_1, ... x_M \}$, with sufficient statistics $\phi_i(\vx) = \delta_i(\vx) = \mathbb{I}(\vx = \vx_i)$ indicating whether the observation $\vx$ matches event $\vx_i$.   We can define each element of the parameter vector $\theta = \{ \theta_1, ... \theta_M \}$ as a difference of $\ln_\qqq$ probabilities, where the final index $\ln_\qqq p(\vx_M)$ enforces normalization.
% \begin{align}
%     \theta_i = \ln_\qqq p(\vx_i) - & \ln_\qqq p(\vx_M) \qquad \psi_\qqq(\theta) = -\ln_\qqq p(\vx_M) \\
%     \pi_\theta(\vx_i) &= \exp_\qqq \{ \theta \cdot \phi(\vx) - \psi(\theta) \} \\
%     &= \exp_\qqq \{ \ln_\qqq p(\vx_i) - \ln_\qqq p(\vx_M) + \ln_\qqq p(\vx_M) \} \\
%     &= p(\vx_i)
% \end{align}
% Thus, for any order $\qqq$, a discrete distribution is a $\qqq$-exponential family.

\subsection{Student-$t$ Distributions and $q$-Exponential Family}
The Student-$t$ distribution appears in hypothesis testing with finite samples, under the assumption that the sample mean follows a Gaussian distribution.   In particular, the degrees of freedom parameter $\nu = n-1$ can be shown to correspond to an order of the $\qqq$-exponential family with $\nu = (3-\qqq) / (\qqq-1)$ (in 1-d), so that the choice of $\qqq$ is linked to the amount of data observed.

We can first write the multivariate Student-$t$ density, specified by a mean vector $\mu$, covariance $\bSig$, and degrees of freedom parameter $\nu$, in $d$ dimensions, as
\begin{align}
    t_{\nu}(\vx | \bmu, \bSig) = \frac{1}{Z(\nu, \bSig)} \big[ 1 + \frac{1}{\nu} (x - \bmu)^T \bSig^{-1} (x-\bmu) \big]^{-\big(\frac{\nu + d }{2}\big)} \label{eq:student}
\end{align}
where $Z(\nu, \bSig) = \Gamma(\frac{\nu+d}{2})/\Gamma(\frac{\nu}{2}) \cdot |\bSig|^{-1/2} \nu^{-\frac{d}{2}} \pi^{-\frac{d}{2}}$.  Note that  $\nu > 0$, so that we only have positive values raised to the $-(\nu+d)/2$ power, and the density is defined on the real line.

The power function in \eqref{eq:student} is already reminiscent of the $\qqq$-exponential, while we have first and second moment sufficient statistics as in the Gaussian case.  We can solve for the exponent, or order parameter $q$, that corresponds to $-(\nu+d)/2$ using $-\big(\frac{\nu + d }{2}\big) = \frac{1}{1-\qqq}$.  This results in the relations
\begin{align}
 \nu = \frac{d - d \qqq +2}{\qqq - 1} \qquad \text{or} \qquad \qqq = \frac{\nu+d+2}{\nu+d}
\end{align}
We can also rewrite the $\nu^{-1} \, (x - \bmu)^T \bSig^{-1} (x-\bmu) $ using natural parameters corresponding to $\{x, x^2\}$ sufficient statistics as in the Gaussian case (see, e.g. \citet{matsuzoe2015deformed} Example 4).

Note that the Student-$t$ distribution has heavier tails than a standard Gaussian, and reduces to a multivariate Gaussian as $\qqq \rightarrow 1$ and $\exp_{\qqq}(u) \rightarrow \exp(u)$.  This corresponds to observing $n\rightarrow \infty$ samples, so that the sample mean and variance approach the ground truth \cite{murphy2007conjugate}. %, which was assumed to follow a Gaussian distribution,

\begin{figure}[t]
    \centering
    \subfigure[$q=0$] {\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \subfigure[$q=0.5$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_09.pdf}}
    \subfigure[$q=0.9$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.2\textwidth]{sections/figs/gif/ridge_18.pdf}}
    \subfigure[$q=1$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_20.pdf}}
    \subfigure[$q=2$]{\includegraphics[trim={0 .1cm 0.25cm 0 },clip,width=0.19\textwidth]{sections/figs/gif/gaussian_2.pdf}}
    \caption{Intermediate densities between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$ for various $q$-paths and 10 equally spaced $\beta$. The path approaches a mixture of Gaussians with  weight $\beta$ at $q=0$.  For the geometric mixture ($q=1$), intermediate $\pi_{\beta}$ stay within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:alpha_path22} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.
    %\caption{Intermediate densities using various $q$-paths between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$, with 10 equally spaced $\beta$. The $q$-path approaches a mixture of Gaussians with mixing parameter $\beta$ at $q=0$.  For the geometric mixture at $q=1$, the path remains within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:gaussian_path} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.\
    \vspace*{-.15cm}
\end{figure}%
\begin{figure}[t]
    \centering
    % \subfigure[$q=0$]{\includegraphics[trim={0 1.2cm 0 1cm},clip,width=0.19\textwidth]{sections/figs/gif/ridge_01.pdf}}
    \includegraphics[trim={0 0 0 0 },clip,width=0.99\textwidth]{sections/figs/student_t.pdf}
    \caption{Intermediate densities between Student-$t$ distributions, $t_{\nu = 1}(-4, 3)$ and $t_{\nu = 1}(4,1)$ for various $q$-paths and 10 equally spaced $\beta$,
    Note that $\nu=1$ corresponds to $q=2$, so that the $q=2$ path stays within the $q$-exponential family.\\[3ex]
    We provide code to reproduce experiments at \url{https://github.com/vmasrani/q\_paths}.
    }
    \label{fig:alpha_path} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.
    %\caption{Intermediate densities using various $q$-paths between $\mathcal{N}(-4, 3)$ and $\mathcal{N}(4,1)$, with 10 equally spaced $\beta$. The $q$-path approaches a mixture of Gaussians with mixing parameter $\beta$ at $q=0$.  For the geometric mixture at $q=1$, the path remains within the exponential family since both $\pi_0$, $\pi_T$ are Gaussian.}
    \label{fig:student_path} %is a geometric mixture paramterized by $\beta$, which corresponds to a path of and becomes a geometric mixture parameterized by $\beta$ at $q=1$.\
    \vspace*{-.15cm}
\end{figure}

\subsection{Annealing between 1-d Student-$t$ Distributions}
Since the Student-$t$ family generalizes the Gaussian distribution to $q \neq 1$, we can run a similar experiment annealing between two Student-$t$ distributions.   We set $q=2$, which corresponds to $\nu = 1$ with $\nu = (3-\qqq) / (\qqq-1)$, and use the same mean and variance as the Gaussian example in Fig. \ref{fig:alpha_path22}, with $\pi_0(z) = t_{\nu=1}( -4, 3)$ and $\pi_1(z) = t_{\nu=1}( 4, 1)$.

We visualize the results in Fig. \ref{fig:student_path}.   For this special case of both endpoint distributions within a parametric family, we can ensure that the $q=2$ path stays within the $q$-exponential family of Student-$t$ distributions.   We make a similar observation for the Gaussian case and $q=1$ in Fig. \ref{fig:gaussian_path}.   Comparing the $q=0.5$ and $q=0.9$ Gaussian path with the $q=1.0$ and $q=1.5$ path, we observe that mixing behavior appears to depend on the relation between the $q$-path parameter and the order of the $q$-exponential family of the endpoints.

As $q \rightarrow \infty$, the power mean \eqref{eq:abstract_mean} approaches the $\min$ operation as $1-q \rightarrow -\infty$.    In the Gaussian case, we see that, even at $q=2$, intermediate densities for all $\beta$ appear to concentrate in regions of low density under both $\pi_0$ and $\pi_T$.   However, for the heavier-tailed Student-$t$ distributions, we must raise the $q$-path parameter significantly to observe similar behavior.


\subsection{Endpoints within a Parametric Family}
If the two endpoints $\pi_0, \tpi_1$ are within a $q$-exponential family, we can show that each intermediate distribution along the $q$-path of the same order is also within this $q$-family.  However, we cannot make such statements for general endpoint distributions or members of  different $q$-exponential families.

\paragraph{Exponential Family Case}
We assume potentially vector valued parameters $\theta = \{ \theta\}_{i=1}^N$ with multiple sufficient statistics $\phi(\vz) = \{ \phi_i(\vz) \}_{i=1}^N$, with $\theta \cdot \phi(\vz) = \sum_{i=1}^N \theta_i \phi_i(\vz)$.
For a common base measure $\base(\vz)$, let $\pi_0(\vz) = \base(\vz) \, \exp\{ \theta_0 \cdot \phi(\vz) \}$ and $\tpi_1(\vz) = \base(\vz) \, \exp \{ \theta_1 \cdot \phi(\vz) \}$.   Taking the geometric mixture,
\begin{align}
    \tpi_\beta(\vz) &= \exp \big\{ (1-\beta) \, \log \pi_0(\vz) + \beta \, \log \tpi_1(\vz) \big\} \\
    &= \exp \big \{ \log \base(\vz) + (1-\beta) \, \theta_0 \cdot \phi(\vz) + \beta  \, \theta_1 \phi(\vz)  \big \} \\
    &= \base(\vz) \exp  \big \{ \big( (1-\beta) \, \theta_0 + \beta  \, \theta_1 \big) \cdot \phi(\vz)  \big \}
\end{align}
which, after normalization, will be a member of the exponential family with natural parameter $(1-\beta) \, \theta_0 + \beta  \, \theta_1$.




\paragraph{$q$-Exponential Family Case} For a common base measure $\base(\vz)$, let $\pi_0(\vz) = \base(\vz) \, \exp_q \{ \theta_0 \cdot \phi(\vz) \}$ and $\tpi_1(\vz) = \base(\vz) \, \exp_q \{ \theta_1 \cdot \phi(\vz) \}$.   The $q$-path intermediate density becomes
\begin{align}
\tilde{\pi}^{(q)}_\beta(\vz) &= \big[ (1-\beta) \, \pi_0(\vz)^{1-q} + \beta \, \tpi_1(\vz)^{1-q} \big]^{\frac{1}{1-q}} \\
&= \big[ (1-\beta) \, \base(\vz)^{1-q} \, \exp_q \{ \theta_0 \cdot \phi(\vz) \}^{1-q} + \beta \, \base(\vz)^{1-q} \,\exp_q \{ \theta_1 \cdot \phi(\vz) \} ^{1-q} \big]^{\frac{1}{1-q}} \\
&=  \bigg[ \base(\vz)^{1-q} \bigg ( (1-\beta) \,  \, [1 + (1-q)( \theta_0 \cdot \phi(\vz))]^{\frac{1}{1-q}1-q} + \beta  \, [1 + (1-q)( \theta_1 \cdot \phi(\vz))]^{\frac{1}{1-q} 1-q} \bigg) \bigg]^{\frac{1}{1-q}} \nonumber \\
&= \base(\vz) \bigg[ 1 + (1-q) \bigg( \big((1-\beta) \, \theta_0 + \beta  \, \theta_1 \big)  \cdot \phi(\vz) \bigg) \bigg]^{\frac{1}{1-q}} \\
&= \base(\vz) \exp_q \big\{  \big((1-\beta) \, \theta_0 + \beta  \, \theta_1 \big) \cdot \phi(\vz) \big\}
\end{align}
which has the form of an unnormalized $q$-exponential family density with parameter $(1-\beta) \, \theta_0 + \beta  \, \theta_1$.
%\begin{align}
%     \tilde{\pi}^{(q)}_\beta(\vz) = \begin{cases}\big[ (1-\beta) \, \pi_0(\vz)^{1-q} + \beta \, \tpi_1(\vz)^{1-q} \big]^{\frac{1}{1-q}} & q \neq 1 \\[1.3ex]
%      \exp \big\{ (1-\beta) \, \log \pi_0(\vz) + \beta \, \log \tpi_1(\vz) \big\} & q = 1  \\[1.25ex]
%     \end{cases},  \label{eq:alpha_mix3}
% \end{align}



==> sections/app/vm_naudts_paths.tex <==
\section{Derivation of Path $q$-Family}\label{app:q_path}
With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
\begin{align}
    \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
\end{align}
which is suggestive of the convex conjugate for $\psi_q$ via
\begin{align}
    \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
\end{align}
We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

\begin{proof}
\begin{align}
    \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
    &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
    &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
\end{align}
Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
\begin{align}
    \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
    Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
\end{align}

To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
\begin{align}
    \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
\end{align}
and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
\begin{align}
    \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
    &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
    &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
\end{align}
where we have defined
\begin{align}
    \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
\end{align}
\end{proof}



\section{Alternative Derivation}
Note that $\exp_q \{ x + y \} = \exp_q \{ y \} \cdot \exp_q \{ \frac{x}{1 + (1-q) y}  \}$ from \textcolor{red}{Vaden's theorem below.}, instead of $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $ for the standard exponential.  This implies that
\begin{align}
\pi_{q,\beta} = \pi_0 \, \exp_q \{ \beta \cdot \phi(\vz) - \psi_q \} &= \pi_0 \, \exp_q\{ -\psi_q \} \exp_q \{ \frac{\beta}{1+(1-q)(-\psi_q)} \cdot \phi(\vz) \} 
\end{align}
Our goal is to express $\pi_{q,\beta}(\vz)$ using a normalization constant $Z$ instead of the $q$-free energy $\psi_q(\beta)$.  While the exponential family allows us to freely move between  $\log Z_{\beta}$
and $\psi(\beta)$, in the $q$-exponential case, we must adjust the parameters.   Defining
%To (w/ $\eta, \beta$ switched) match Naudts, let : }
\begin{align}
 \eta &= \frac{\beta}{1+(1-q)(-\psi_q)} \\
Z_q(\eta) &= \frac{1}{\exp_q \{-\psi_q \}} := \exp_{q}^{*}\{ -\psi_q\} \\
\end{align}
we obtain a new parameterization of the $q$-exponential family, using parameters $\eta$ and multiplicative normalization constant $Z_q(\eta)$, as
\begin{align}
 \pi_{q,\beta} =  \pi_{q,\eta} &=  \frac{1}{Z_q(\eta)} \exp_{q} \{ \eta \cdot \phi(\vz) \}
\end{align}
See \citet{matsuzoe2019normalization} for more detailed discussion of normalization in deformed exponential families.


==> sections/app/vm_q_sum_prod.tex <==
\section{Sum and Product Identities for $q$-Exponentials}\label{app:q_sum_product}
In this section, we prove two lemmas which are useful for manipulation expressions involving $q$-exponentials, for example in moving between \cref{eq:normalization1} and \cref{eq:normalization2} in either direction.
\begin{lemma}
    Sum identity
    \begin{align}
        \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
    \end{align}
    \label{lemma:q_exp_sum}
\end{lemma}
\begin{lemma}
    Product identity
    \begin{align}
        \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
    \end{align}
    \label{lemma:q_exp_prod}
\end{lemma}

\subsection{Proof of \cref{lemma:q_exp_sum}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
    \begin{align}
        \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \left[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \right]_{+}^{1/(1-q)} \\
                                                &= \left[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \right]_{+}^{1/(1-q)} \\
                                                &= \left[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \right]_{+}^{1/(1-q)} \\
                                                &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
                                                &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
    \end{align}
\end{proof}
\subsection{Proof of \cref{lemma:q_exp_prod}}
\begin{proof}
    We prove by induction. The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + = (1 - q)x_i\right)$. Then, 
    %and $(1-q) = (1 - q)$. Then
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
    &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \hspace*{-.5cm} \text{(reindex $n \to n - 1)$} \nonumber \\
    &=\exp_q(x_{0})\exp_q(y_N) & \hspace*{-.5cm} \text{(inductive hypothesis)} \nonumber \\
    &= \bigg[\left(1 + (1-q) \cdot x_{0}\right)\left(1 + (1-q) \cdot y_N\right) \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \cdot x_{0} + \big(1 + (1-q) \cdot x_{0} \big)(1-q) \cdot y_N \bigg]_{+}^{1/(1-q)}\\
    &= \bigg[1 + (1-q) \bigg(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\bigg) \bigg]_{+}^{1/(1-q)}\\
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)y_N\right)
\end{align}
Next we use the definition of $y_N$ and rearrange
\begin{align}
    &= \exp_q \left(x_{0} + \big(1 + (1-q) \cdot x_{0} \big)\left(x_1 + x_2(1 + (1-q) \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + (1-q) \cdot x_i)\right)\right) \nonumber\\
    &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q) x_i\right)\right).
\end{align}
Then reindexing $n \to n + 1$ establishes
\begin{align}
    \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1-q)x_i\right)\right).
\end{align}
\end{proof}


% \section{Sum Identity for $q$-exponentials}\label{app:q_sum_product}
% %\section{Sum and product identities for $q$-exponentials}\label{app:q_sum_product}
% While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $, this is not true for $\exp_{\alpha}\{ x + y \}$.   We derive a more general expression for the $q$-exponential below.
% %In the Lemma below, prove a more general statement for the $q$-exponential.
% %We therefore derive two lemmas for q-exponentials which will be useful in obtaining the $q$-exponential family. We will prove both statements by induction and simplify notation by defining $(1-q) := 1 - q$.

% \begin{lemma}
%     Sum identity
%     \begin{align}
%         \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$ so that the denominator on the \textsc{rhs} of \cref{eq:q_exp_sum} is $1$. Assuming \cref{eq:q_exp_sum} holds for $N$,
%         \begin{align}
%             \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + (1-q) \sum_{n=1}^{N+1} x_n \bigg]^{1/(1-q)} \\
%                                                     &= \bigg[ 1 + (1-q) \left(\sum_{n=1}^{N} x_n\right) + (1-q)x_{N+1} \bigg]^{1/(1-q)} \\
%                                                     &= \bigg[\left( 1 + (1-q) \sum_{n=1}^{N} x_n \right) \left(1 + (1-q)\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n}\right) \bigg]^{1/(1-q)} \\
%                                                     &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + (1-q) \sum_{n=1}^{N} x_n} \right)\\
%                                                     &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + (1-q)\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
%         \end{align}
%     \end{proof}
% \end{lemma}

% %\section{Sum and product identities for $q$-exponentials}\label{app:q_sum_product}
% While the exponential family has the convenient property that $\exp \{ x + y \} = \exp \{ x \} \cdot \exp \{ y \} $, this is not true for $\exp_{\alpha}\{ x + y \}$. We therefore derive two lemmas for q-exponentials which will be useful in obtaining the $q$-exponential family. We will prove both statements by induction and simplify notation by defining $\bar{q} := 1 - q$.

% \begin{lemma}
%     Sum identity
%     \begin{align}
%         \exp_q\left(\sum_{n=1}^N x_n\right) = \prod_{n=1}^{N} \exp_q \left(\frac{x_n}{1 + (1 - q)\sum_{i=1}^{n-1}x_i} \right)\label{eq:q_exp_sum}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\sum_{i=a}^bx_i = 0$ if $b < a$. Assuming \cref{eq:q_exp_sum} holds for $N$,
%         \begin{align}
%             \exp_q\left(\sum_{n=1}^{N+1} x_n\right) &= \bigg[ 1 + \bar{q} \sum_{n=1}^{N+1} x_n \bigg]^{1/\bar{q}} \\
%                                                     &= \bigg[ 1 + \bar{q} \left(\sum_{n=1}^{N} x_n\right) + \bar{q}x_{N+1} \bigg]^{1/\bar{q}} \\
%                                                     &= \bigg[\left( 1 + \bar{q} \sum_{n=1}^{N} x_n \right) \left(1 + \bar{q}\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n}\right) \bigg]^{1/\bar{q}} \\
%                                                     &= \exp_q\left(\sum_{n=1}^N x_n\right) \exp_q \left(\frac{x_{N+1}}{1 + \bar{q} \sum_{n=1}^{N} x_n} \right)\\
%                                                     &= \prod_{n=1}^{N+1} \exp_q \left(\frac{x_n}{1 + \bar{q}\sum_{i=1}^{n-1}x_i} \right) \text{(using the inductive hypothesis)}
%         \end{align}
%     \end{proof}
% \end{lemma}

% \begin{lemma}
%     Product identity
%     \begin{align}
%         \prod_{n=1}^N \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + (1 - q)x_i\right)\right)\label{eq:q_exp_prod}
%     \end{align}
%     \begin{proof}
%         The base case ($N=1$) is satisfied using the convention $\prod_{i=a}^bx_i = 1$ if $b < a$. Assuming \cref{eq:q_exp_prod} holds for $N$, we will show the $N+1$ case. To simplify notation we define $y_N:=\sum_{n=1}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)$. Then
%     \begin{align}
%         \prod_{n=1}^{N+1} \exp_q(x_n) &= \exp_q(x_{1})\left(\prod_{n=2}^{N+1}\exp_q(x_n)\right)\\
%         &= \exp_q(x_{0})\left(\prod_{n=1}^{N}\exp_q(x_n)\right) & \text{(reindex $n \to n - 1)$}\\
%         &=\exp_q(x_{0})\exp_q(y_N) & \text{(inductive hypothesis)}\\
%         &= \bigg[\left(1 + \bar{q} \cdot x_{0}\right)\left(1 + \bar{q} \cdot y_N\right) \bigg]^{1/\bar{q}}\\
%         &= \bigg[1 + \bar{q} \cdot x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\bar{q} \cdot y_N \bigg]^{1/\bar{q}}\\
%         &= \bigg[1 + \bar{q} \bigg(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\bigg) \bigg]^{1/\bar{q}}\\
%         &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)y_N\right)
%     \end{align}
%     Next we use the definition of $y_N$ and rearrange
%     \begin{align}
%         &= \exp_q \left(x_{0} + \big(1 + \bar{q} \cdot x_{0} \big)\left(x_1 + x_2(1 + \bar{q} \cdot x_1) + ... + x_N \cdot \prod_{i=1}^{N-1}(1 + \bar{q} \cdot x_i)\right)\right)\\
%         &= \exp_q\left(\sum_{n=0}^{N}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q} x_i\right)\right).
%     \end{align}
%     Then reindexing $n \to n + 1$ establishes
%     \begin{align}
%         \prod_{n=1}^{N+1} \exp_q(x_n) = \exp_q\left(\sum_{n=1}^{N+1}x_n \cdot \prod_{i=1}^{n-1} \left(1 + \bar{q}x_i\right)\right).
%     \end{align}
% \end{proof}
% \end{lemma}







% \section{Derivation of Path $q$-Family}\label{app:q_path}
% \vm{This longer derivation is necessary to establish relationship between two q-exp fam forms and allow for tvo/ti trick. Might also be better to save for full paper and revert to prev}
% With normalization, the $q$-exponential family is usually written as %= \exp_{\alpha}\{ x \}* \exp_{\alpha}\{ y \}$
% \begin{align}
%     \pi_{t,q}(\z)  &= \pi_0(z) \, \exp_q \big\{ \eta \cdot \phi(\vz) - \psi_q(\eta)  \big\} \label{eq:lnq_fam_form1}
% \end{align}
% which is suggestive of the convex conjugate for $\psi_q$ via
% \begin{align}
%     \ln_q \frac{\pi_{t,q}(\z) }{\pi_0(z)} =  \eta \cdot \phi(\vz) - \psi_q(\eta)
% \end{align}
% We now derive the $q$-exponential family from the $\alpha$ mixture between $\pi_0$ and $\pi_1$, where we will obtain sufficient statistics of $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$.

% \begin{proof}
% \begin{align}
%     \pi_{\alpha, \beta}(z) &\propto \bigg[(1 - \beta) \pi_0^{1 - \alpha} + \beta\pi_1^{1 - \alpha}\bigg]^\frac{1}{1 - \alpha}\\
%     &= \bigg[\pi_0^{1 - \alpha} + \beta\big(\pi_1^{1 - \alpha} - \pi_0^{1 - \alpha}\big)\bigg]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \left[1 + \beta\left(\left(\frac{\pi_1}{\pi_0}\right)^{1 - \alpha} - 1\right)\right]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \left[1 + (1-\alpha)\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right]^\frac{1}{1 - \alpha}\\
%     &= \pi_0 \exp_\alpha\left[\beta\ln_\alpha\left(\frac{\pi_1}{\pi_0}\right)\right].
% \end{align}
% Defining $\phi(\vz) = \ln_{q} \frac{\pi_1(\z)}{\pi_0(\z)}$ and normalizing, we arrive at
% \begin{align}
%     \pi_{\alpha, \beta}(z) = \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \quad
%     Z_\alpha(\beta) &:= \int dz \pi_0 \exp_\alpha\left[\beta \phi(\vz) \right].\label{eq:lnq_fam_form2}
% \end{align}

% To get \cref{eq:lnq_fam_form2} into the standard $q$-exponential family form, we define
% \begin{align}
%     \psi_\alpha := \ln_\alpha^* \left(Z_\alpha(\beta)\right) \label{eq:psi_alpha}
% \end{align}
% and rewrite \cref{eq:lnq_fam_form2} using \cref{eq:q_exp_prod}
% \begin{align}
%     \pi_{\alpha, \beta}(z) &= \frac{\pi_0}{Z_\alpha(\beta)}\exp_\alpha\left[\beta \phi(\vz) \right] \\
%     &= \frac{\pi_0}{\exp^*_\alpha\left(\psi_\alpha\right)}\exp_\alpha\left(\beta \phi(\vz) \right) & \text{Using  \cref{eq:psi_alpha}}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha\right) \exp_\alpha\left(\beta \phi(\vz)\right) & \text{Using $\exp^*_\alpha(u) = 1/\exp_\alpha(-u)$}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \bigg(1 - (1 - \alpha) \psi_\alpha\bigg)\beta\phi(\vz)\right) & \text{Using \cref{eq:q_exp_prod}}\\
%     &= \pi_0 \exp_\alpha\left(-\psi_\alpha + \eta \phi(\vz)\right)
% \end{align}
% where we have defined
% \begin{align}
%     \eta := \beta \cdot \big(1 - (1 - \alpha) \psi_\alpha\big).
% \end{align}
% \end{proof}

